Hybrid-IoT: Hybrid Blockchain Architecture for Internet of Things - PoW Sub-blockchains

From its early days the Internet of Things (IoT) has evolved into a decentralized system of cooperating smart objects with the requirement, among others, of achieving distributed consensus. Yet, current IoT platform solutions are centralized cloud based computing infrastructures, manifesting a number of significant disadvantages, such as, among others, high cloud server maintenance costs, weakness for supporting time-critical IoT applications, security and trust issues. Enabling blockchain technology into IoT can help to achieve a proper distributed consensus based IoT system that overcomes those disadvantages. While this is an ideal match, it is still a challenging endeavor. In this paper we take a first step towards that goal by designing Hybrid-IoT, a hybrid blockchain architecture for IoT. In Hybrid-IoT, subgroups of IoT devices form PoW blockchains, referred to as PoW sub-blockchains. Then, the connection among the PoW sub-blockchains employs a BFT inter-connector framework, such as Polkadot or Cosmos. In this paper we focus on the PoW sub-blockchains formation, guided by a set of guidelines based on a set of dimensions, metrics and bounds. In order to prove the validity of the approach we carry a performance and security evaluation.

==> DEPRECATED.tex <==
As per Section \ref{sec:architecture}, light peer devices send transactions to full peer devices, and those will include them in the newly generated blocks.
Hence, the first type of experiment that we run to test performance is a stress test, in which a full peer device DoSed by twenty light peer devices that are continuously sending transactions to it (see Section \ref{sec:perfEva1}).
Then, we shift the focus to the generation of sub-blockchains that contain different number of full peer devices.
In that, we monitor performance and resource usage of the full peer devices in different sized sub-blockchains (see Section \ref{sec:perfEva2}).




\begin{figure*} 
    \centering
   \subfloat[Perf Eva \rom{1}: CPU Light peer device]{%
     \includegraphics[width=0.5\linewidth]{figures/LightCPU.png}}
     \label{1a} \hfill
  \subfloat[Perf Eva \rom{1}: CPU Full peer device]{%
      \includegraphics[width=0.5\linewidth]{figures/20LiDOS.png}}
     \label{1b} \hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{1}]{%      
     \includegraphics[width=0.33\linewidth]{figures/20liYeni.png}}
  	  \label{1c}
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{2}]{%
      \includegraphics[width=0.33\linewidth]{figures/40liYeni.png}}
    \label{1d}\hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{3}]{%
      \includegraphics[width=0.33\linewidth]{figures/100luYeni.png}}
     \label{1e}\hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{4}]{%
      \includegraphics[width=0.33\linewidth]{figures/200luYeni.png}}
     \label{1f} 
  \caption{CPU utilization of devices in Performance Evaluation \rom{1} and \rom{2}}
  \label{fig:CpuUtil} 
\end{figure*}





ARCHITECTURE
8 MARCH DEPRECATED:
%The key challenge for successful integration is the limited transaction throughputs of PoW-based blockchains.
%In fact, the more devices become blockchain peers, the higher transaction throughput must be achieved.
%Hybrid-IoT achieves high ratio of the transaction throughput to number of devices by having multiple PoW-based sub-blockchains generated according to sweet-spot settings defined in Section \ref{sec:sweetspot}.
%Sub-blockchains have to be connected to each other in order to achieve interoperability.
%
%Particularly, full peer devices include inter-blockchain transactions to the newly generated blocks in their sub-blockchain.
%Then, inter-blockchain transactions transferred to the one node of the BFT-based blockchain connector framework that is assigned for its sub-blockchain.
%
%High transaction processing abilities of BFT-based consensus protocols\footnote{Tendermint protocol used by Cosmos network able to process thousands of transactions per second \cite{tendermint}}, let them to scale many sub-blockchains by processing their inter-blockchain transactions.
%In fact, PoW-based sub-blockchains able to process few dozens of transactions per second and presumably only sub-set of their transactions will be inter-blockchain transactions and processed by blockchain connector framework.
%This is very convenient in order to scale to many sub-blockchains, as sub-blockchains are able to process few dozens of transactions according to our evaluations presented in Section \ref{sec:integrationEva}.
%Moreover, presumably only sub-set of transactions in sub-blockchains will be inter-blockchain transactions and send to the blockchain connector framework.


%In parallel to this role, today's blockchain protocols offer simple blockchain client models.
%For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{\url{en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}} and send transactions %without block mining or downloading the entire copy of the blockchain. 




SECURITY
8 MARCH DEPRECATED
%The more work a  PoW-based blockchain contains, the more secure it is against threats targeting its integrity, as noted in Section \ref{sec:metrics}.
%Yet in Hybrid-IoT, we propose to divide IoT devices into subgroups and form sub-blockchains.
%Clearly, if total work in each sub-blockchain decreases, it would be easier for a malicious party to generate a longer blockchain and destroy data accountability and integrity.
%By frequent block generation and low stale block generation rates, sub-blockchains may be as robust as the unique blockchain.
%In the following, we quantitatively analyze total work that both unique blockchains contain and sub-blockchains contain, by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings} for 100 minutes of system execution.


..
..
..
2 li versiyon
\iffalse
%\textbf{Hybrid-IoT.} 
%One of the biggest challenges in the integration of blockchain into IoT ecosystems is scalability.
%In fact, due to the massive number of devices and resource constraints, employing blockchain mechanisms in IoT is particularly challenging.
%The optimal blockchain architecture has to scale to many IoT devices (they become the peers on the blockchain network), and it should be able to process a high throughput of transactions.
%To this end, in this paper we propose a hybrid blockchain architecture, that we call Hybrid-IoT. 
%Hybrid-IoT exploits both PoW-based and BFT-based blockchains.
%First, PoW-based blockchains are used to achieve distributed consensus among many IoT devices as being blockchain peers.
%We define a set of PoW-based blockchain-IoT integration metrics that clarify prerequisites of successful deployment.
%We observed that, by forming multiple PoW-based sub-blockchains that are containing few hundreds of IoT devices that are geographically close to each other, high performance (i.e. high transaction throughputs and low block propagation delays) can be achieved.
%Given that, Hybrid-IoT leverages on a BFT-based multiple blockchain connector framework such as Polkadot\footnote{polkadot.network} and Cosmos\footnote{cosmos.network} in order to achieve interoperability among sub-blockchains.


%\textbf{This work.}
%In this paper, as a first step, we focus on the challenging issue of adapting PoW-based blockchains to the IoT domain by generating sub-blockchains.
%In fact, generating sub-blockchains is not a straightforward task, where both performance and security properties of sub-blockchains have to be considered.
%ELENA: explain what sweet spot setting is
%GOKHAN: Rewritten.
%To this end, we define set of PoW-based blockchain-IoT integration metrics to clarify prerequisites of successful deployment evaluate performance.
%By exploiting the integration metrics we evaluate performance of the integration and by varying block sizes and block generation intervals, device locations, and number of devices as blockchain peers.
%According to our observations, we define a set of rules to regulate sub-blockchain generation without sacrificing security properties, referred to as sweet-spot settings.
%We define the Hybrid-IoT architecture with three roles for IoT devices.
%Moreover, we evaluate the performance of IoT devices with regards to their roles by performing stress test and varying sub-blockchain sizes.
\fi



..
..
..
eski versiyon
\iffalse
%One of the biggest challenges in the integration of blockchain into IoT ecosystems is scalability.
%In fact, due to the massive number of devices and resource constraints, employing blockchain mechanisms in IoT is particularly challenging.
%The optimal blockchain architecture has to scale to many IoT devices (they become the peers on the blockchain network), and it should be able to process a high throughput of transactions.
%To this end, in this paper we propose a hybrid blockchain architecture, that we call Hybrid-IoT. Hybrid-IoT exploits both PoW-based and BFT-based blockchains.
%First, PoW-based blockchains are used to achieve distributed consensus among many IoT devices as being blockchain peers.
%(\textbf{THE PART BELOW I DO NOT UNDERSTAND AND I CANNOT SEE ITS POINT})
%We extensively evaluated performance of the PoW-blockchains in IoT setting in order to assess best practices.
%In that, we observed that blockchains containing few hundreds of IoT devices that are geographically close to each other achieve high performance.
%Given that, Hybrid-IoT includes multiple PoW-blockchains, referred to as sub-blockchains, and a BFT-based multiple blockchain connector framework such as Polkadot\footnote{polkadot.network} and Cosmos\footnote{cosmos.network} in order to achieve interoperability among sub-blockchains.
..
..
..
%\textbf{This work.} In this paper, as a first step, we focus on the challenging issue of adapting PoW-based blockchains to the IoT domain by generating sub-blockchains.
%In fact, generating sub-blockchains is not a straightforward task, where both performance and security properties of sub-blockchains have to be considered.
%As such, we have to achieve high performance with high transaction throughputs and low block propagation delays.
%To this end, we propose a set of rules in generating sub-blockchains to achieve high performance, without sacrificing security properties, referred to as sweet-spot settings.
%(\textbf{PERFORMANCE NEEDS TO BE DEFINED}) 
% GOKHAN: Done.
%By exploiting sub-blockchain approach we design the Hybrid-IoT architecture.
%Moreover, we have defined three roles for IoT devices with regards to their capabilities. 
%(\textbf{SHOULD BE MORE PRECISE BELOW, AKA... WE DO CERTAIN TYPE OF EXPERIMENTS TO EVALUATE AND DESCRIBE THEM BRIEFLY})
%We extensively evaluate performance of generating sub-blockchains by varying block sizes and block generation intervals, device locations, and number of devices as blockchain peers.
%Moreover, 
%and security of generating sub-blockchains, by  
%We extensively evaluate performance and security of generating sub-blockchains, by  
\fi




%Sweet-spot settings:  IoT devices that are geographically close to each other and frequently communicating with each other should be in the same sub-blockchain, sub-blockchains should contain neither too few nor too many IoT devices, key blockchain system parameters, i.e. block size and block generation interval, should be set in such a way that ensures to achieve low stale block generation rates and high decentralization degrees.





ARCHITECTURE


\iffalse
We have to connect sub-blockchains to each other.
To this end, Hybrid-IoT exploits a  BFT-based multiple blockchain connector framework such as Polkadot and Cosmos to perform secure and trust-free inter-blockchain transactions.
We present an example of Hybrid-IoT architecture containing two sub-blockchains in Figure \ref{fig:architecture}.
The main advantage of using BFT-based blockchain as a multiple blockchain connector is achieving high transaction throughputs with low latencies \cite{blockchainSurvey}.
Transaction throughputs of the PoW-based sub-blockchains will be much less than the BFT-based multiple-blockchain connector framework. 
Moreover, presumably only sub-set of transactions in sub-blockchains will be inter-blockchain transactions and send to the connector framework.
As long as connector framework is able to execute and transmit inter-blockchain transactions with very low latency, adding new sub-blockchains generated with the sweet-spot settings do not overwhelm and degrade execution in the Hybrid-IoT. 
Therefore, each new sub-blockchain can preserve its ratio of the transaction throughput to number of devices.
Given that, we claim that, Hybrid-IoT achieves linear scalability in number of devices and transaction throughput of the system.
%\footnote{ripple.com/dev-blog/ripple-consensus-ledger-can-sustain-1000-transactions-per-second}

 \begin{figure*} [h] 
	\centering
	\includegraphics[width=\textwidth]{figures/newArchitecture.png}
	\caption{Hybrid-IoT} \label{fig:architecture}
\end{figure*}
\fi





\iffalse
%In that, in Hybrid-IoT, devices with different capabilities take different roles.
In order to group IoT devices on some common blocks and identify device roles in blockchain systems, we refer to the IoT device classification presented in \cite{ourPaper2}. 
In \cite{ourPaper2}, IoT devices, aka smart objects, have been classified into three groups according to their capabilities, referred to as smartness levels, namely; first, second, and third smartness levels.
At the first smartness level, IoT devices have a very limited capacity by being able only to act as basic sensors, for sensing data from the environment.
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors.
%like Complex Event Processing (CEP) systems.
At the second smartness level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply), such as Arduino Yun.
Whereas, at the third smartness level, devices have enough capacity and computing power for performing more complex operations by their own, such as Raspberry Pi Model B.
\fi


%\textbf{Motivations} : 
%\textbf{Transparency and accountability} As discussed previously, blockchain is replicated among every peer and newly generated blocks are shared to the network. As such, blockchain technology offers great transparency. Recording every transaction ensures accountability, as such blockchain data structure is kind of ledger containing history of every operation performed that are visible to all parties participating (in public blockchains they are publicly visible).  

%We propose to integrate blockchain technology into IoT domain by exploiting its foundational properties to solve some important problems of the IoT domain. 

DECENTRAZLIATION, SECURITY, GLOBAL IDENTIFICATION
By having the potential to solve crucial problems of the IoT domain, foundational properties of the blockchain technology, such as its tamper-proof and decentralized nature and strong security, offers great promises for IoT domain.
Such foundational properties give shape to proposed multi blockchain architecture. 
%Let us discuss how blockchain technology fits to IoT domain by listing beneficial foundational properties of the blockchain technology and how they can help IoT domain in the following as \textit{security, decentralization, transparency} and \textit{identification}.




%Cryptography forms a central part of blockchain protocols. 
%Cryptography is used to protect the integrity of the blockchain, where every block of the blockchain contains a hash of the previous block. 
%Changing contents of a block requires the modification of all following blocks. 
%Additionally, all popular blockchains use \textit{Digital signature algorithms} to cryptographically sign transactions sent among peers, specifically the Elliptic Curve Digital Signature Algorithm (ECDSA) is used to authenticate transactions. 

%\textbf{Security}
%Since blockchain technology uses cryptography for data and transaction encryption, even  every peer of the network has all blockchain data and able to compute everything, the underlying meaning of the information is completely obfuscated from original data\footnote{blog.ethereum.org/2016/01/15/privacy-on-the-blockchain/}.
%Considering security issues that we are facing today in IoT domain, such as unsecured communication among devices and poor authentication of IoT devices, foundational properties of blockchain technology may improve integrity and authenticity of the IoT applications. 
%In Section \ref{sec:security} we analyze and test security properties of proposed architecture.  



%\textbf{Decentralization} 
%Blockchain technology is a peer to peer decentralized technology, without a centralized intermediary. 
%Peers of the network agree on the state of the blockchain by achieving consensus, which overcomes the problem of a single point of failure. 
%Indeed, assuming majority of the peers of the network are active and honest, blockchain ensures that even if some peers drop out temporarily from the network, consensus among honest peers will be achieved. 
%Considering today's IoT, where IoT is evolving into a loosely coupled, decentralized system of cooperating smart objects, we have to consider the IoT domain as independent objects with the ability to cooperate without knowing or trusting each other. The decentralized nature of blockchain technology is a great fit for today's smart objects. 



\textbf{Resource restricted IoT Devices} 
IoT devices show great diversity regarding their capabilities \cite{Nistir, ourPaper2,ituStandard}. 
Devices with low processing capabilities and storage space will be cumbersome for integration of blockchain technology into IoT domain. 
As we discuss in \ref{sec:architecture}, we propose to use multiple blockchains to decrease resource usage of blockchain protocols. 
Additionally, we propose the use of light blockchain protocols to increase collaboration of resource restricted devices in blockchain systems, where we showed performance results in Section \label{sec:lightPerformance}.

%\textbf{Ever changing needs of IoT domain}
%IoT technology is expanding and changing very fast, therefore new uses emerges according to that. Previously discussed smart contract concept with increased programming capabilities of blockchains, e.g. Ethereum, offers great promises to overcome such challenges. Indeed, we propose to use of smart contract concept of blockchain technology in order to perform complex use cases with proposed architecture.
%\textbf{Protection and security of devices}
%IoT devices with poor authentication and authorization mechanisms generates important vulnerabilities to any system. In Section \ref{sec:security} we discuss security threats to proposed architecture in detail, how they may effect the system and how to protect system against such threats.
%\textbf{Limited monitoring and lack of standards on IoT devices} Today, many IoT Systems are poorly designed and implemented with different protocols and technologies\footnote{www.iot.ieee.org/newsletter/january-2017/iot-and-blockchain-convergence-benefits-and-challenges.html}. Additionally, there is limited guidance for life cycle management of IoT device and lack of standards. Therefore, we propose a flexible blockchain architecture, where blockchain protocols 





\iffalse
%d


%Massive number of IoT devices, expected to be around twenty billions, according to ITU \cite{ituIoT}, is an important issue that gives rise to serious concerns for the future of the domain. 
%Additionally, Device and data security, data accountability and device identification of IoT systems always in question and mostly very fragile and weak. 
%Indeed, considering growth of the IoT market and newly interconnected devices increase attack surface simply because each of them can become the weakest link and exploited \cite{learningIoTsecurity}. 


\subsection{Evaluation \rom{4}: Cost of the Proof of Work Consensus}\label{sec:eva4}
In order to solve the PoW puzzle, miner devices have to use their resources (e.g. in case of Bitcoin CPU/GPU) and use electricity.
In what follows, we discuss cost of the PoW consensus algorithm, on an example case of Bitcoin by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings}. 
Bitcoin miners perform double SHA-256 functions to take hash of the string representing transactions and a nonce \cite{bitcoinEnergy}. 
Hashing operation is repeated by varying the nonce value until a hash result less then the pre-defined target value has been found.
In Bitcoin blockchain, difficulty is used to regulate target value according to total hash power in the Bitcoin network to have 10 minutes average block generation interval.
With total hash rate of $HR$ and difficulty $Diff$, the formula\footnote{en.bitcoin.it/wiki/Difficulty} to calculate the expected time to find a new block $T_{E}$ is:

\begin{align}
T_{E} \approx \frac{Diff * {2^{32}}}{HR}    
\end{align}


Based on this formula, we evaluate the cost, difficulty and hash rate relation of Bitcoin's PoW algorithm on IoT domain. 
We have used Raspberry Pi Model B \footnote{www.raspberrypi.org/products/raspberry-pi-1-model-b/} as a reference IoT device to calculate it's electricity consumption cost. 
Single Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and uses 3.5 watts of electricity per hour (3.5 W/h)\footnote{$en.bitcoin.it/wiki/Non specialized_hardware_comparison$}.
We picked the Netherlands as a reference country in calculating electricity costs.
In the Netherlands electricity cost is around 0.20\$ for kilo watts per hour(KW/h)\footnote{$ec.europa.eu/eurostat/statistics-explained/index.php/Electricity_price_statistics$} for household usage.
Let us first present the relation of number of devices to total hash power and electricity cost on system execution for one day in Figure \ref{fig:cost1}.
Total hash power in the system and electricity consumption costs of IoT devices change in direct proportion to number of devices in the system.


\begin{figure} [H]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/deviceHashCost.png}
	\caption{Cost - difficulty relation \label{fig:cost1}}
\end{figure}


Secondly, we evaluate the relation of cost, block generation interval and network latency (nodes' location) to generate 10000 blocks with 500 KB size.  
To this end, we refer to experiment results presented in Evaluation \rom{2}, that demonstrates number of blocks generated in 100 minutes of system execution in different location settings (the Netherlands, Europe, World).
We present cost analysis results in Table \ref{tab:costAnalysis}.

\begin{table}  
\centering
\begin{tabular} {|c|cc|cc|cc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Interval:} & \multicolumn{2}{c}{\textbf{Netherlands}} & \multicolumn{2}{c}{\textbf{Europe}} & \multicolumn{2}{c}{\textbf{World}} \\
\cmidrule(lr){2-3}  
\cmidrule(lr){4-5} 
\cmidrule(lr){6-7} 
\textbf{Results/} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$}  \\
\textbf{Cases}	  & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$}  & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$}\\
\midrule
\textbf{10 minutes}   & 1.81 					& 0\%        					&  1.81  						&0\% 						& 1.97						&  0\%\\ 
\hline
\textbf{5 minutes}   &  1.32					& 0\%        					&  1.32  						&0\% 						& 1.40						&  0\%\\ 
\hline
\textbf{1 minute}   &  0.21						& 1.76\%        				&  0.24							&5.14\% 					& 0.24						&  8.22\%\\  
\hline
\textbf{30 seconds}   &  0.13					& 5.15\%        				&  0.13							&  12.87\% 					& 0.14						& 14.11\%\\ 
\hline
\textbf{10 seconds}   &  0.09					& 32.49\%        			    &  0.10 						&  33.31\% 					& 0.12						&  41.34\%\\ 
\hline
\textbf{5 seconds}   &  0.14					& 47.66\%        				&  0.15							&  51.80\% 					& 0.16						&  53.12\%\\ 
\bottomrule             
\end{tabular}
\caption{Cost analysis} \label{tab:costAnalysis} 
\end{table}


First important aspect to examine is the total cost.
We have observed that, with shorter block generation intervals total costs are less as devices have to operate less amount of time to produce 1000 blocks.
However, in 5 seconds setting due to very high stale block rate, total cost is higher than 10 seconds and 30 seconds setting.
In evaluating total cost of the system, another important aspect to consider besides total cost of the energy waste. 
Energy spent to generate and propagate a stale block have to be considered as a waste of energy, as stale blocks do not included to blockchain. 
Shorter block generation intervals imply higher stale block generation rates, and thus higher waste of energy.
For example, in 5 seconds block generation interval setting, stale block generation rates for all location settings are around 50\%.
This signifies that around half of the consumed electricity and thus total cost is unutilized.
Thus, such systems are very inefficient, and they do not comply with the efficiency metric. 
As discussed in Evaluation \rom{2}, the Netherlands setting shows the lowest stale block generation rates and thus the most efficient and cheapest setting. 
Given all, we conclude that, short block generation intervals in low network latency settings with low stale rates should be used for maximum energy efficiency and low electricity costs.











%d
\subsection{Evaluation \rom{5}: Blockchain types}\label{sec:eva5}
Today, different types of blockchains are in use to address requirements of different businesses and domains.
Blockchains are mostly categorized into three groups as; \textit{public, private} and \textit{consortium} blockchains.
Public blockchains referred as permissionless blockchains, whereas private and consortium blockchains are referred as permissioned blockchains.
Blockchains in different groups show great difference in terms of their methodology to achieve consensus and rights assigned to the blockchain nodes.
In the following, we evaluate different types of blockchains regarding whether they are suitable for IoT domain or not.


\subsubsection{Public blockchains}\label{sec:publicBlc}
In public blockchains,any device with an active internet connection can send transactions, read the blockchain, and take part in the consensus process.
Public blockchains do not depend on central authority or trusted entity, and they are close to be fully decentralized. 
As long as majority of the mining power in the network is acting honestly, malicious parties can not divert the blockchain.
However, IoT devices have limited resources and thus limited mining powers, and this is a problem in designing public blockchain.
In example case of Bitcoin, Raspberry Pi, has 0.2 MH/s mining power\footnote{$en.bitcoin.it/wiki/Non specialized_hardware_comparison$}, whereas a specialized mining device AntMiner S9 \footnote{www.amazon.com/Bitmain-Antminer-S9-Bitcoin-Efficiency/dp/B075MH4HSL} has 14 GH/s mining power.
That means, even a single specialized mining hardware con oppress millions of standard IoT devices, and may forge system to operate maliciously. 
Given that, public blockchain is not suitable for IoT domain.


\subsubsection{Private blockchains}\label{sec:privateBlc}
In private blockchains, right of writing to the blockchain and participating in the consensus process is only kept to one entity, whereas read access may be public or may be given to some entities with limited context. 
As consensus process is handled by one trusted source, malicious parties with specialized hardwares can not divert blockchain actions like as in public blockchains.
To divert a private PoW blockchain, attacker has to both gain access to miner devices and have the majority of the hashrate. % to ensure its blocks are generated faster than the rest of the network combined.
Private blockchains offer much faster block generation and confirmation times, as device faults can be corrected manually and devices are supposed to be very well connected. 
Furthermore, the entity that is running private blockchain can change blockchain rules easily and divert malicious activities.
However, this will cause big problems against cooperation of different parties as only one party is in charge of consensus and others have to trust the authority.
Indeed, private blockchains are centralized and they lack trustless communication and cooperation of different parties which is one of the biggest advantages of using blockchain technology.
Given all, we conclude that, private blockchains offer some advantages and thus can be suitable for some IoT use-cases, however they lack some important features of public blockchains like decentralization.


\subsubsection{Consortium blockchains}\label{sec:consortiumBlc}
In consortium blockchains, writing to the blockchain and taking part in the consensus process is distributed into set of nodes, whereas read access may be given to some entities with limited context or it may be public.  
Subset of nodes from different parties can be authorized to write to the blockchain and take part in consensus process.
By doing so, all parties take part in the consensus process, and as long as majority of the mare honest,they can protect the integrity of the blockchain from dishonest parties.
Similar with private blockchains, attacker both needs to gain access to pre-selected authorized nodes on consensus and have the majority of the mining power to maliciously alter the blockchain.
In contrast to private blockchains, partial decentralization in consortium blockchains allow cooperation of different parties. 
In consortium blockchains, sybil resistance to off-chain can be increased by holding mining power in trusted resources.
Ideally, all parties should contribute to consensus process with equal mining power to achieve decentralization and communicate without trust. 
Even though consortium blockchains does not provide fully decentralized consensus, they allow cooperation of different parties with less security threats from malicious parties.   
Given all, we conclude that, consortium blockchains can be a suitable solution in designing an IoT application containing various parties as services providers or device vendors.
%The way people try to use PoW for consortium networks does not cause excess power usage: low difficulty, low powered device/s.








%d
\subsection{Evaluation \rom{6}: IoT devices as blockchain nodes}\label{sec:eva6}
In IoT domain, device capabilities are extremely heterogeneous.
To group IoT devices on some common blocks, we refer to the device classification based on their capabilities as presented in \cite{ourPaper2}.
In \cite{ourPaper2}, smartness of the IoT devices, aka smart objects, have been classified into three smartness levels as; first, second, and third smartness levels.
In the following, we examine how IoT devices that are classified into different smartness levels can be part of the blockchain. 


\subsubsection{First smartness level -- Sensors}\label{sec:firstLevelDevice} 
At the first level, devices have a very limited capacity, being able only to act as  basic sensors, for sensing data from the environment.   
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors like Complex Event Processing (CEP) systems.
Thus, such devices can not be peers in the blockchain network. 
The ideal way to somehow connect those devices to the blockchain network is connecting them to other devices that are peers of the blockchain network. 
If we consider many sensors that are continuously sensing raw data, storing all raw data in the blockchain will be a big hurdle against scalability of the blockchain system.
Therefore, raw data sent by sensors should be processed by higher capability devices or data processing systems that are peers of the blockchain network.
Sensor data needs to be stored in the cloud or servers.
Peers, however, may form transactions and send it to the blockchain network after data processing, if required.
Given all, devices with first smartness level can not directly participate in blockchains, but they can connect to smarter intermediary device indirectly participate.

\subsubsection{Second smartness level -- Devices with low capabilities}\label{sec:secondLevelDevice} 
At the second level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply).
For example, Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be categorized as a device with second level smartness.
Those devices are able to run basic operating systems such as Alpine Linux\footnote{alpinelinux.org}, and they can connect to the blockchain network.
As such devices run am operating systems and able to process data, they can participate in the blockchain network by performing some simple tasks, like sending transactions.
In parallel with that, today's blockchain protocols offer simple client models.
For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}.
Thin clients perform simpler operations like sending transactions and thus require less resources. 
As such, thin clients do not download all blockchain but they download a complete copy of the headers for all blocks in the entire blockchain and they do not participate in the consensus process.
Given all, devices with second smartness level can take simple client roles that do not require to mine blocks are participate in consensus process, like thin client role in case of Bitcoin. 


\subsubsection{Third smartness level -- Devices with high capabilities}\label{sec:thirdLevelDevice} 
At the third level, devices have enough capacity and computing power for performing more complex operations by their own.
For example, Raspberry Pi Model B\footnote{raspberrypi.org/products/raspberry-pi-1-model-b} can be categorized as a device with third level smartness.
Those devices run more advanced operating systems like Raspbian\footnote{www.raspbian.org}, and they are able to connect and participate in the blockchain network. 
Such devices can perform more complex blockchain tasks than devices with lower smartness level, such as mining blocks and taking part in the consensus process. 
However, their capabilities are not enough to solve very complex PoW puzzles to mine a block, or propagate big blocks.
For example, in case of Bitcoin, Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and with the difficulty setting in Bitcoin network in late 2017, it would take more than 1000 years to solve the PoW puzzle for a million Raspberry Pi Bs.
Moreover, their bandwidth capabilities are limited, therefore very big block sizes or very short block generation interval settings are not suitable for such devices (as discussed in Evaluation \rom{1}).
Given all, devices with the third level of smartness can participate in the blockchain networks as full peers, by carefully setting consensus parameters and blockchain rules such as block size and block generation interval.

\fi


















%Since inter-chain transactions affect current status of both of the blockchains, and to preserve integrity and accountability, inter-chain transactions will be recorded by multiple blockchain connector framework, presumably in its local blockchain (as its done in Polkadot\cite{polkadot}). As such, overall system traceability and consensus will be ensured.
\iffalse
\textbf{Multichain connector framework: }
\textbf{polakdot.}
Polkadot \cite{polkadot}. presents a vision for heterogeneous multi-chain framework. 
In this framework, rather than presenting a single chain, Polkadot provides the bedrock \textit{relay-chain} upon which a large number of blockchains may be hosted (called as \textit{parachains}). In Polkadot, relay chain will have its own security and security will be shared across the parachains(blockchains that are connected to the Polkadot framework). Polkadot provides trust-free transactions between independent parachains. Polkadot framework provides trust free bridges allowing transactions to be routed from a parachain to another. Polkadot parachains communicates via interchain communication, so they have some sort of communication channel between them. 

Polkadot network consists four basic roles to keep up the network, namely \textit{Validator}, \textit{Nominator}, \textit{Collator} and \textit{Fisherman}.
Validator helps seal new block on the Polkadot network, which refers to relay chain and all parachains. 
A Validator must run a relay-chain implementation with high availability and bandwidth, in order to be ready to accept new block on a nominated parachain. 
Validator receives the block from nominated parachain, validates it, and then republishes the block. 
%Validation of a block requires fully-synchronized database of the parachain, but since maintaining all of the parachains is not reasonable, validator will nominate the task of devising a suggested new parachain block to collator. 
Firstly, validator subgroups validates all new parachain blocks, then validators must ratify the relay-chain block itself
. 
A validator is punished if it does not act honestly or does not fulfill its duty to find consensus.  
Nominator is a stake-holding party contributing security bond of a validator. 
Nominators select validators that they trust to act responsibly in maintenance of the network, and they place risk capital to such validator. 
%They receive increase or decrease in their deposit according to the bond's growth.
Collator assists validator in producing valid parachain blocks. 
Collators maintain a "full-node" in particular parachain, meaning that they can retain all information required to author new blocks and execute transactions. Collator executes transactions to create unsealed block and provides the block to the validators with zero-knowledge proof.    
Fishermen is not an active part and does not take role in block authoring process. Fishermen, are independent "bounty-hunters", they get their reward by proving one bonded party acted illegally.

Polkadot achieves low-level consensus over a set of mutually agreed and valid block through asynchronous \textit{Byzantine Fault Tolerant (BFT)} algorithm. 
Polkadot determines set of validators and incentives validators by utilizing \textit{Proof of Stake (PoS)} based selection criteria. 
In Polkadot, parachains' header are sealed within the relay-chain block ensuring no reorganisation or "double-spending" is possible after confirmation of block. 
Additionally, Polkadot also provides strong guaranty that the state transitions of parachains are valid.  Polkadot parachains communicates via interchain communication, so they have some sort of communication channel between them.


Cosmos [10] is a proposed multi-chain system in the
same vein as side-chains, it describes multiple chains (operating in
zones) each using individual instances of Tendermint, together
with a means for trust-free communication via a
master hub chain.
This interchain communication is limited
to the transfer of digital assets ( about tokens")
rather than arbitrary information, however such interchain
communication does have a return path for data,
e.g. to report to the sender on the status of the transfer.
Validator sets for the zoned chains, and in particular
the means of incentivising them, are, like side-chains, left
as an unsolved problem. The general assumption is that
each zoned chain will itself hold a token of value whose in-

ation is used to pay for validators. Still in the early stages
of design, at present the proposal lacks comprehensive details
over the economic means of achieving the scalable
certainty over global validity. However, the loose coherence
required between the zones and the hub will allow
for additional 
exibility over the parameters of the zoned
chains compared to that of a system enforcing stronger
coherence.
\fi






































LOCATION EXPERIMENTS
\iffalse
%Netherlands
\begin{table} 
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.65}           & \textbf{0.00} 	     &{\bf 9.65} 			  &  {\bf 0.0\%}	 & {\bf 7.13}   & {\bf 13.37}    & {\bf 3.21 TX/s}  \\
        \hline
         \textbf{5 minutes}		 & {\bf 18.65}          & \textbf{0.00} 		 &{\bf 18.65}  			  &  {\bf 0.0\%} 	 & {\bf 6.89}   & {\bf 26.74}    & {\bf 6.21 TX/s}  \\
        \hline
         \textbf{1 minutes}		 & {\bf 92.14}          & \textbf{0.66} 	     &{\bf 91.48}     		  &  {\bf 0.71\%} 	 & {\bf 9.11}   & {\bf 136.45}      & {\bf 30.71 TX/s} \\
        \hline
         \textbf{30 seconds} 	 & {\bf 165.20}         & \textbf{2.59} 	     &{\bf 162.61}            &  {\bf 1.56\%}    & {\bf 20.45}   & {\bf 499.78}      & {\bf 54.2 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 346.58}         & \textbf{101.39} 	     &{\bf 245.19}            &  {\bf 29.25\%}   & {\bf 314.08}   & {\bf 14762.93}     & {\bf 81.73 TX/s} \\
        \hline 
         \textbf{5 seconds} 	 & {\bf 350.68}         & \textbf{161.18} 	     &{\bf 189.50}            &  {\bf 45.96\%}   & {\bf 815.39}  & {\bf 41378.1}     & {\bf 63.16 TX/s} \\
        \hline       
    \end{tabular}
\caption{Evaluation \rom{1} Netherlands cities setting} \label{tab:eva2Netherlands}
\end{table}

%Europe
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.96} 			& \textbf{0} 		     &{\bf 9.96}  			  &  {\bf 0\%}	     & {\bf 16.69s}     & {\bf 13.54}  &{\bf 3.32 TX/s}\\
        \hline
         \textbf{5 minutes}		 & {\bf 16.39}		    & \textbf{0}		     &{\bf 16.39}  			  &  {\bf 0\%} 		 & {\bf 13.62s}     & {\bf 27.92}  &{\bf 5.46 TX/s}\\
        \hline
         \textbf{1 minutes}		 & {\bf 93.6} 			& \textbf{4.82} 		 &{\bf 88.78}     		  &  {\bf 5.14\%} 	 & {\bf 14.32s}     & {\bf 140.06}  &{\bf 29.59 TX/s}\\
        \hline
         \textbf{30 seconds} 	 & {\bf 170.54}         & \textbf{21.94} 	     &{\bf 148.6}             &  {\bf 12.87\%}   & {\bf 38.55s}     & {\bf 527.75}  &{\bf 49.53 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 314.04}         &\textbf{104.60} 	     &{\bf 209.44}            & {\bf 33.31\%}    & {\bf 355.99s}    & {\bf 15237.3} &{\bf 69.81 TX/s}\\
        \hline 
         \textbf{5 seconds} 	 & {\bf 301.25}         &\textbf{156.04}         &{\bf 145.21}            & {\bf 51.80\%}    & {\bf 918.98s}    & {\bf 43931.4} &{\bf 37.83 TX/s}\\
        \hline       
    \end{tabular}
\caption{Europe cities setting} \label{tab:eva2Europe}
\end{table}

%World
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.96} 			& \textbf{0} 		     &{\bf 10.96}  			  &  {\bf 0\%}	     & {\bf 20.03s}    & {\bf 13.64}	 &{\bf 3.32 TX/s}\\
        \hline
         \textbf{5 minutes}		 & {\bf 15.45}		    & \textbf{0}		     &{\bf 15.45}  			  &  {\bf 0\%} 	     & {\bf 17.73s}    & {\bf 27.46}     &{\bf 5.15 TX/s}\\
        \hline
         \textbf{1 minutes}		 & {\bf 96.52} 		    & \textbf{7.93} 		 &{\bf 88.59}     		  &  {\bf 8.22\%} 	 & {\bf 20.85s}    & {\bf 140.78}    &{\bf 29.53 TX/s}\\
        \hline
         \textbf{30 seconds} 	 & {\bf 169.46}         & \textbf{23.91} 	     &{\bf 145.55}            &  {\bf 14.11\%}   & {\bf 52.1s}     & {\bf 592.76}    &{\bf 48.51 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 331}            &\textbf{136.83} 	     &{\bf 194.17}            &  {\bf 41.34\%}   & {\bf 392.74s}   & {\bf 16777.5}   &{\bf 64.72 TX/s}\\
        \hline 
         \textbf{5 seconds} 	 & {\bf 303.28}         &\textbf{161.1}         &{\bf 142.18}             &  {\bf 53.12\%}   & {\bf 1000.49s}   & {\bf 45021.32} &{\bf 47.39 TX/s}\\
        \hline        
    \end{tabular}
\caption{World cities setting} \label{tab:eva2World}
\end{table}

\fi











time - size experiments

  
\iffalse
\begin{table}
    \centering
    \scriptsize
    \begin{tabular} {*{8}{c}} %{|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 10.82} 			& \textbf{0.00} 		 &{\bf 10.82}  			  &  {\bf 0.00\%}	 & {\bf 156.77}  &{\bf 276.50}  & {\bf 72.13}  \\
         
         
        \hline
         \textbf{5 MB}		 & {\bf 10.27}		    & \textbf{0.00}		     &{\bf 10.27}  			  &  {\bf 0.00\%} 	 & {\bf 78.35}   &{\bf 134.08} & {\bf 34.23}  \\
        \hline
         \textbf{1 MB}		 & {\bf 12.33} 			& \textbf{0.00} 		 &{\bf 12.33}     		  &  {\bf 0.00\%} 	 & {\bf 14.32}   &{\bf 26.64} & {\bf 8.22} \\
        \hline
         \textbf{500 KB} 	 & {\bf 9.65}           & \textbf{0.00} 	     &{\bf 9.65}              &  {\bf 0.00\%}    & {\bf 7.13}    &{\bf 13.37}  & {\bf 3.21}\\
        \hline
         \textbf{100 KB}     & {\bf 9.33}           & \textbf{0.00} 	     &{\bf 9.33}              &  {\bf 0.00\%}    & {\bf 1.48}    &{\bf 2.74} & {\bf 0.62} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 11.00}          & \textbf{0.00}          &{\bf 11.00}             &  {\bf 0.00\%}    & {\bf 0.72}    &{\bf 1.41} & {\bf 0.36} \\
        \hline      
         \textbf{10 KB}      & {\bf 10.33}          & \textbf{0.00}          &{\bf 10.33}             &  {\bf 0.00\%}    & {\bf 0.17}    &{\bf 0.34} & {\bf 0.06}  \\
        \hline    
    \end{tabular}
\caption{10 minutes block generation interval setting} \label{tab:10min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 18.84} 			& \textbf{0.91} 		 &{\bf 17.93}  			  &  {\bf 4.83\%}	 & {\bf 201.01} 	 &{\bf 723.40}  & {\bf 119.53}  \\
        \hline
         \textbf{5 MB}		 & {\bf 19.97}		    & \textbf{0.66}		     &{\bf 19.31}  			  &  {\bf 3.30\%} 	 & {\bf 91.73}      &{\bf 288.10}  & {\bf 64.36}  \\
        \hline
         \textbf{1 MB}		 & {\bf 22.33} 			& \textbf{0.00} 		 &{\bf 22.33}     		  &  {\bf 0.00\%} 	 & {\bf 15.44}    	 &{\bf 53.28}   & {\bf 14.88} \\
        \hline
         \textbf{500 KB} 	 & {\bf 18.65}          & \textbf{0.00} 		 &{\bf 18.65}     		  &  {\bf 0.00\%}    & {\bf 6.89}       &{\bf 26.74}   & {\bf 6.21}\\
        \hline
         \textbf{100 KB}     & {\bf 23.00}          & \textbf{0.00} 		 &{\bf 23.00}     		  &  {\bf 0.00\%}    & {\bf 1.46}       &{\bf 5.48}    & {\bf 1.53} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 18.66}          & \textbf{0.00} 		 &{\bf 18.66}     		  &  {\bf 0.00\%}    & {\bf 0.74}       &{\bf 2.82}   & {\bf 0.62} \\
        \hline      
         \textbf{10 KB}      & {\bf 21.66}          & \textbf{0.00} 		 &{\bf 21.66}     		  &  {\bf 0.00\%}    & {\bf 0.17}       &{\bf 0.69}   & {\bf 0.14}  \\
        \hline    
    \end{tabular}
\caption{5 minutes block generation interval setting} \label{tab:5min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 45.65} 			& \textbf{16.02} 		 &{\bf 26.93}  			  &  {\bf 35.07\%}	 & {\bf 618.57}   	 &{\bf 21215.86}    & {\bf 197.53}  \\
        \hline
         \textbf{5 MB}		 & {\bf 67.30}		    & \textbf{12.11}		 &{\bf 55.19}  			  &  {\bf 17.99\%} 	 & {\bf 214.97}     &{\bf 8718.29}   & {\bf 183.96}  \\
        \hline
         \textbf{1 MB}		 & {\bf 92.47} 			& \textbf{0.66} 		 &{\bf 91.81}     		  &  {\bf 0.71\%} 	 & {\bf 31.95}    	 &{\bf 438.86} & {\bf 61.20} \\
        \hline
         \textbf{500 KB} 	 & {\bf 92.14}          & \textbf{0.66} 	     &{\bf 91.48}             &  {\bf 0.71\%}    & {\bf 9.11}       &{\bf 136.45}  & {\bf 30.71}\\
        \hline
         \textbf{100 KB}     & {\bf 99.00}           &\textbf{0.00} 	     &{\bf 99.00}             &  {\bf 0.00\%}    & {\bf 1.47}       &{\bf 27.40}   & {\bf 6.6} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 96.33}           &\textbf{0.00} 	     &{\bf 96.33}             &  {\bf 0.00\%}    & {\bf 0.76}       &{\bf 14.12}   & {\bf 3.21} \\
        \hline      
         \textbf{10 KB}      & {\bf 101.00}          &\textbf{0.00} 	     &{\bf 101.00}            &  {\bf 0.00\%}    & {\bf 0.17}      &{\bf 3.49}    & {\bf 0.67}  \\
        \hline    
    \end{tabular}
\caption{1 minute block generation interval setting} \label{tab:1min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 51.28} 			& \textbf{26.67} 		 &{\bf 24.61}  			  &  {\bf 47.99\%}	 & {\bf 1154.07}   &{\bf 49520.10}  & {\bf 164.06}  \\
        \hline
         \textbf{5 MB}		 & {\bf 73.49}		    & \textbf{26.84}		 &{\bf 46.65}  			  &  {\bf 36.52\%} 	 & {\bf 657.17}   	 &{\bf 28528.53}  & {\bf 155.5}  \\
        \hline
         \textbf{1 MB}		 & {\bf 165.91}			& \textbf{8.56} 		 &{\bf 157.35}     		  &  {\bf 5.15\%} 	 & {\bf 52.26}   	 &{\bf 3243.78}  & {\bf 104.9} \\
        \hline
         \textbf{500 KB} 	 & {\bf 165.20}         & \textbf{2.59} 	     &{\bf 162.61}            &  {\bf 1.56\%}    & {\bf 20.45}      &{\bf 639.78} & {\bf 54.2}\\
        \hline
         \textbf{100 KB}     & {\bf 186.41}         &\textbf{0.66} 	         &{\bf 185.75}            &  {\bf 0.35\%}    & {\bf 1.49}       &{\bf 54.85}   & {\bf 12.38} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 187.00}         &\textbf{0.66}           &{\bf 186.34}            &  {\bf 0.35\%}    & {\bf 0.75}       &{\bf 28.24}   & {\bf 6.21} \\
        \hline      
         \textbf{10 KB}      & {\bf 193.33}         &\textbf{0.0}            &{\bf 193.33}            &  {\bf 0.00\%}   & {\bf 0.17}        &{\bf 6.99}   & {\bf 1.28}  \\
        \hline    
    \end{tabular}
\caption{30 seconds block generation interval setting} \label{tab:30sec}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 57.77} 			& \textbf{41.24} 		 &{\bf 16.53}  			  &  {\bf 71.38\%}	 & {\bf 1732.54} &{\bf 151046.00}  & {\bf 110.2}  \\
        \hline
         \textbf{5 MB}		 & {\bf 84.09}		    & \textbf{56.5}		     &{\bf 27.59}  			  &  {\bf 67.18\%} 	 & {\bf 1486.55} &{\bf 100255.03}   & {\bf 91.96}  \\
        \hline
         \textbf{1 MB}		 & {\bf 219.69}         & \textbf{94.18} 		 &{\bf 125.51}     		  &  {\bf 42.86\%} 	 & {\bf 693.22}  &{\bf 30259.26}   & {\bf 83.67} \\
        \hline
         \textbf{500 KB} 	 & {\bf 346.58}         & \textbf{101.39} 	     &{\bf 245.19}            &  {\bf 29.25\%}   & {\bf 314.08}  &{\bf 14762.93}  & {\bf 81.73}\\
        \hline
         \textbf{100 KB}     & {\bf 537.31}         & \textbf{6.21} 	     &{\bf 531.1}             &  {\bf 1.15\%}    & {\bf 5.50}     &{\bf 447.74} &{\bf 35.4} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 562.00}         & \textbf{4.66}          &{\bf 557.33}            &  {\bf 0.82\%}    & {\bf 0.77}    &{\bf 84.55}  & {\bf 18.57} \\
        \hline      
         \textbf{10 KB}      & {\bf 598.66}         & \textbf{0.00}          &{\bf 598.66}            &  {\bf 0.00\%}    & {\bf 0.17}    &{\bf 20.94}   & {\bf 3.99}  \\
        \hline    
    \end{tabular}
\caption{10 seconds block generation interval setting} \label{tab:10sec}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 64.26} 			& \textbf{48.20} 		 &{\bf 16.06}  			  &  {\bf 75.00\%}	 & {\bf 1988.84}  &{\bf 273777.66}  & {\bf 107.06}  \\
        \hline
         \textbf{5 MB}		 & {\bf 91.42}		    & \textbf{68.49}		 &{\bf 22.93}  			  &  {\bf 74.91\%} 	 & {\bf 1738.58}  &{\bf 190671.00}  & {\bf 76.43}  \\
        \hline
         \textbf{1 MB}		 & {\bf 232.52} 		& \textbf{128.7} 		 &{\bf 103.87}     		  &  {\bf 55.37\%} 	 & {\bf 1105.55}  &{\bf 69059.33}  & {\bf 69.24} \\
        \hline
         \textbf{500 KB} 	 & {\bf 350.68}         & \textbf{161.18} 	     &{\bf 189.50}            &  {\bf 45.96\%}   & {\bf 815.39}   &{\bf 41378.10}   & {\bf 63.16}\\
        \hline
         \textbf{100 KB}     & {\bf 954.55}         &\textbf{124.51} 	     &{\bf 830.04}            &  {\bf 13.04\%}   & {\bf 57.48}    &{\bf 7249.57}   & {\bf 55.33} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 1120.39}        &\textbf{9.79}           &{\bf 1110.60}           &  {\bf 0.87\%}    & {\bf 4.25}     &{\bf 931.01} & {\bf 37.02} \\
        \hline      
         \textbf{10 KB}      & {\bf 1166.30}        &\textbf{2.33}           &{\bf 1163.97}           &  {\bf 0.19\%}    & {\bf 0.18}     &{\bf 41.94}   & {\bf 7.75}  \\
        \hline    
    \end{tabular}
\caption{5 seconds block generation interval setting} \label{tab:5sec}
\end{table}
\fi









Varying no




\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		   &{\bf 9H}  	 		    &{\bf 12H}	   		    &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
       \hline
    \end{tabular}
\caption{Fixed difficulty settings} \label{tab:fixedDifficultySettings}
\end{table}


\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{29.96}     &\textbf{0}	   &\textbf{29.96}    &  {\bf 0\%}	    &\textbf{7.85}           &{\bf 44.17}      & {\bf 9.86}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{76.67}     &\textbf{1.33}	   &\textbf{75.34}	  &  {\bf 1.73\%}	 &\textbf{7.97}          &{\bf 88.9}       & {\bf 25.11}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{101.29}     &\textbf{1.8}	    &\textbf{99.49}	  &  {\bf 1.77\%}	 &\textbf{8.07}          &{\bf 134.51}     & {\bf33.16}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{177.67}     &\textbf{20.59}	    &\textbf{157.08}	  &  {\bf 11.52\%}	  &\textbf{41.19}     &{\bf 1168.86}& {\bf 52.36}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{237.18}     &\textbf{32.90}	    &\textbf{204.28}	  &  {\bf 13.87\%}	  &\textbf{147.13}     &{\bf 3485.49}& {\bf 68.09}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{216.45}     &\textbf{39.39}	    &\textbf{177.06}	  &  {\bf 18.2\%}	  &\textbf{291.87}     &{\bf 5791.87}& {\bf 59.02}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{211.98}     &\textbf{47.55}	    &\textbf{164.43}	  &  {\bf 22.43\%}	  &\textbf{498.97}     &{\bf 8265.55}& {\bf 54.81}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3 - Fixed difficulty setting} \label{tab:case3.1}
\end{table}









\iffalse
%Req analysis ten kontrol et, bi kismi orda artik.
\textbf{IoT devices as blockchain peers} We propose the use of different roles as blockchain peers for IoT devices, considering resource heterogeneity of IoT device ecosystem.
To do so, we propose to use two main roles \textbf{full peers} and \textbf{light peers}. 
As such, IoT devices as full peers will be responsible for transaction validation, block generation, participating in consensus and maintaining all or recent block of the local blockchain.
Whereas light peers, will likely to be able to only receive and send transactions to other devices. 
IoT devices that have limited resources, like CPU power, memory and bandwidth will participate in blockchain networks as light peers, since participation in resource intensive operations like consensus might overwhelm the device. 
For example, IoT devices like Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be used for monitoring and performing basic operations, can take the light peer role, where more advanced devices like Raspberry Pi 3 B \footnote{raspberrypi.org/products/raspberry-pi-3-model-b/}, that are able to perform more resource intensive tasks, may take the full peer role. 
Two main roles, full and light peers, might be diversified by regulating resource usage and participation to the blockchain operations. 
Today's blockchain protocols offers different client models for their protocols, like in Bitcoin as full clients and thin clients\footnote{www.en.bitcoin.it/wiki/Clients}, which we adopted to our Bitcoin emulation to evaluate resource need in Section \ref{sec:emulation}.  
\fi



smartness - device -smartness level

....
In IoT domain, device capabilities are extremely heterogeneous.
To group IoT devices on some common blocks, we refer to the device classification based on their capabilities as presented in \cite{ourPaper2}.
In \cite{ourPaper2}, smartness of the IoT devices, aka smart objects, have been classified into three smartness levels as; first, second, and third smartness levels.
In the following, we examine how IoT devices that are classified into different smartness levels can be part of the blockchain. 


\textbf{First smartness level -- Sensors}\label{sec:firstLevelDevice} 
At the first level, devices have a very limited capacity, being able only to act as  basic sensors, for sensing data from the environment.   
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors like Complex Event Processing (CEP) systems.
Thus, such devices can not be peers in the blockchain network. 
The ideal way to somehow connect those devices to the blockchain network is connecting them to other devices that are peers of the blockchain network. 
If we consider many sensors that are continuously sensing raw data, storing all raw data in the blockchain will be a big hurdle against scalability of the blockchain system.
Therefore, raw data sent by sensors should be processed by higher capability devices or data processing systems that are peers of the blockchain network.
Sensor data needs to be stored in the cloud or servers.
Peers, however, may form transactions and send it to the blockchain network after data processing, if required.
Given all, devices with first smartness level can not directly participate in blockchains, but they can connect to smarter intermediary device indirectly participate.

\textbf{Second smartness level -- Devices with low capabilities}\label{sec:secondLevelDevice} 
At the second level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply).
For example, Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be categorized as a device with second level smartness.
Those devices are able to run basic operating systems such as Alpine Linux\footnote{alpinelinux.org}, and they can connect to the blockchain network.
As such devices run am operating systems and able to process data, they can participate in the blockchain network by performing some simple tasks, like sending transactions.
In parallel with that, today's blockchain protocols offer simple client models.
For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}.
Thin clients perform simpler operations like sending transactions and thus require less resources. 
As such, thin clients do not download all blockchain but they download a complete copy of the headers for all blocks in the entire blockchain and they do not participate in the consensus process.
Given all, devices with second smartness level can take simple client roles that do not require to mine blocks are participate in consensus process, like thin client role in case of Bitcoin. 


\textbf{Third smartness level -- Devices with high capabilities}\label{sec:thirdLevelDevice} 
At the third level, devices have enough capacity and computing power for performing more complex operations by their own.
For example, Raspberry Pi Model B\footnote{raspberrypi.org/products/raspberry-pi-1-model-b} can be categorized as a device with third level smartness.
Those devices run more advanced operating systems like Raspbian\footnote{www.raspbian.org}, and they are able to connect and participate in the blockchain network. 
Such devices can perform more complex blockchain tasks than devices with lower smartness level, such as mining blocks and taking part in the consensus process. 
However, their capabilities are not enough to solve very complex PoW puzzles to mine a block, or propagate big blocks.
For example, in case of Bitcoin, Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and with the difficulty setting in Bitcoin network in late 2017, it would take more than 1000 years to solve the PoW puzzle for a million Raspberry Pi Bs.
Moreover, their bandwidth capabilities are limited, therefore very big block sizes or very short block generation interval settings are not suitable for such devices (as discussed in Evaluation \rom{1}).
Given all, devices with the third level of smartness can participate in the blockchain networks as full peers, by carefully setting consensus parameters and blockchain rules such as block size and block generation interval.





























\textbf{Smart contract concept}  Today, some blockchains use an important concept referred to as "smart contracts". This refers to executable scripts stored in blockchain. The smart contract concept was first introduced in \cite{szabo} as 'a computerized transaction protocol that executes the terms of a contract'. More specifically, smart contracts are deterministic self-executing contractual clauses. Once a smart contract is deployed on a blockchain it is stored forever with the following properties: nobody can control or modify it, it has a unique address. Since smart contracts can not be modified throughout their existence on the blockchain, every peer in the network can trust them. They have unique address on the blockchain, and its clauses can be triggered by peers, by sending transactions to execute them. Smart contracts describe  outcomes of the contract execution and allows us to express business logic inside the blockchain \cite{scForIoT}, which opens up an opportunity for IoT applications.



%d
\subsection{Mining Cartel Attack (51\% attack}\label{sec:51attack}
In mining cartel attack, attacker gathers massive hashrate, that is bigger than 50\% of the total mining power of the devices in the system \cite{miningCartel}.
In performing such attack, and will be able to control the network. 
As such, as long as attacker maintains majority of the mining power in the system, attacker can prevent others to generate new blocks, prevent other devices' transactions to make into blocks.
This attack is a huge threat against robustness of the blockchain, as attacker is able to perform malicious activities and can not be stopped by honest devices.
In our architecture, we suggest to use of consortium or private blockchains (cfr. to Section\ref{sec:background} for more information) would limit this attack factor, as only selected devices can contribute to the block mining process.
However, attacker may compromise devices that are authorized to generate block and if he/she has gathers majority of the mining power, can launch this attack.
We discuss device device compromise attacks in Section \ref{sec:deviceComp}.
In case of mining cartel attack on private or consortium blockchain, firstly, administrators of the blockchain should identify infected devices that are generating malicious transactions and blocks.
Then, honest devices should not propagate blocks and transactions that are sent by infected devices and they should be forced drop their connections to malicious devices.
Finally, the blockchain have to be diverted to the latest correct state before the launching of the attack in all devices by deleting malicious blocks.




%d
\subsection{Device compromise attacks}\label{sec:devComp}
In performing device compromise attacks, attacker subversively gains access to an IoT device, where he can drop the device from the network and may control it to perform malicious activities.
Major threats on blockchains systems related to node compromise attacks are \textit{device capture} and \textit{device controlling}. 
By performing device capture attack, attacker may drop the device from the blockchain network.
In which, device is unable to participate in the network as such; it can not processes data and generate transactions, propagate and check correctness of the blocks and transactions sent by its peer devices.  
Whereas in performing device controlling attack, an attacker may send malicious transactions and blocks, or he/she may use compromised devices to launch other types of attacks, such as mining cartel attack, or Denial of Service (DoS) attack.
IoT devices should be complemented with authentication and authorization mechanisms (see e.g., \cite{authorizationIoT}) and strong passwords to hinder attacker's access to devices.
However, some IoT devices have very limited resources (devices within the first smartness level, see Section \ref{sec:Background}), and they may not be suitable to be complemented with authorization and authentication mechanism.
To cope with device compromise attacks on low level devices, IoT devices with higher capabilities (devices within the third smartness level) should be complemented with intrusion detection systems (see e.g., \cite{intrusionSvelte}, \cite{adversaryNodeCapWSN})  so as  to make them able to analyze the network and detect compromised devices and drop connections.  




%d
\subsection{Sybil attacks}
Sybil attacks refer to maliciously manipulating IoT systems with many sybil IoT devices that are generated with stolen and fabricated identities \cite{sybilDefenceEvaluation}. 
In performing sybil attacks, an attacker node claims several stolen identities, and attempts to fill the blockchain network with clients controlled by him.
In blockchain systems, honest IoT devices may only be connected to sybil devices controlled by the attacker.
Sybil attacks can be performed to disseminate spam and malware to honest smart objects \cite{sybilIoT}.
In PoW blockchains, to generate a block what matters is the computational power, but not the number of entities by count.
In which, as long as attacker has the limited mining power, he would not be able to produce more blocks by generating creating several identities as he distributes his mining power to the his sybil identities.
However, launching a sybil attack can be helpful in executing other attacks, such as network partitioning and eclipse attacks\footnote{www.en.bitcoin.it/wiki/Weaknesses} , that are discussed in Section \ref{sec:networkEclipse}.
In which, by launching sybil attack, victim device would likely to be connected to sybil nodes, thus it gets disconnected from the network. 
By doing that attacker may generate partition the network, or can try to send bogus blocks or transactions to the victim node. 

In IoT domain, various approaches have been proposed to deal with sybil attacks, such as cryptography based approaches \cite{sybilCryptography}, intrusion detection approaches \cite{intrusionSvelte}, or network based approaches making use of RSS readings \cite{rssiSybil,sybilDetection}. 
In order to cope with sybil attacks, IoT devices should be complemented with an hybrid prevention setting, that makes use of both intrusion detection and RSS readings based approaches. 
In particular, IoT devices within third smartness level can be complemented with intrusion detection systems \cite{intrusionSvelte} to detect sybils, as we assume they are honest and have enough resources to host intrusion detection systems. 
Whereas, all IoT devices objects will be complemented with RSS readings based approach \cite{rssiSybil,sybilDetection}, as they offer efficient solutions for resource constrained devices.
Such approaches define a threshold value on RSS readings to distinguish legitimate and sybil nodes based on nodes’ behavior in the network.
In our architecture, we propose to distribute IoT devices into different blockchains by considering their geographical locations to be as close to each other as possible. 
In which, IoT devices will maintain lists of devices and RSS values of devices that are in their coverage area, and they will define a threshold value to detect sybil devices.

%If there is a discrepancy between the amount of work that the two connected nodes claim, then a client knows that the one with the least work is probably doing something malicious, lying.
%providing white-listed devices to the peers; before connecting to the new peer, IoT device should ask for some information from its local blockchain like current difficulty, or information about transactions  or blocks that have been in longest chain for a long time.





%d
\subsection{Network partitioning and Eclipse attacks}\label{sec:networkEclipse}
%eclipse
In eclipse attack on the blockchain systems \cite{eclipseAttack}, attacker monopolizes all of the victim devices' incoming and outgoing connections to the other devices (e.g., 117 to 8 in Bitcoin).
The IP addresses to which the victim IoT device connects are blocked or diverted towards an adversary devices \cite{eclipseAttack}.
Attacker can hold multiple IP addresses, such as by performing sybil attack,and spoof the victim IoT devices from the network.
If all connections of an IoT device are with attacker's malicious devices, attacker may send false blocks and transactions to target IoT devices where victim device have to accept if they are in consistence with device's local blockchain.
However attacker can not force target IoT devices to accept something that network hasn't agreed upon before.


%partitioning
Attacker may try to eclipse set of devices from the rest of the network to generate partitions in the network, referred as network partitioning attack.
In performing network partitioning attack, attacker aims to completely disconnect a set of nodes from the network such that there is no active connection between them \cite{routingAttacks}.
To partition the network, attacker either eclipse victim devices by divert all connections to his sybil identities, or he should cut all the connections by dropping any packets to or from victim device set.
This attack cause to generate more than one subnetworks, where devices in the disjoint parts will have different views of the blockchains and recent transactions.
In which, total hash power of the system will reduce, and victim devices will be forced to waste computational power and energy on obsolete views of blockchain and it might damage correct execution of IoT applications.


%defence
In order to prevent these attacks, IoT devices should be complemented with an hybrid prevention setting, that makes use of both includes white-listed devices method and intrusion detection approach. 
Firstly, IoT devices within third smartness level can be complemented with intrusion detection systems \cite{intrusionSvelte} in order to detect misbehaving devices. 
Moreover, IoT devices should have a list of devices, aka white-listed devices, to store the addresses of trustworthy devices \cite{routingAttacks}. 
Trustiness of the devices should be changed according to activities of the device, in which misbehaving devices detected by intrusion mechanism should be updated as untrusted device, its' connections should be dropped. 







\subsection{Man in the middle (MITM) attack}
In performing attacks targeting communication between IoT devices on blockchain infrastructure, attacker may aim to position herself in between two parties to alter communication by changing transactions and blocks, or to slow down block propagation. Major threats of MITM attack to proposed mechanism are \textbf{data tampering} and \textbf{slowing information propagation}.

\textbf{Data tampering} This attack aims to violate integrity of the transaction by tampering with its data. As discussed in Section \label{sec:background}, blockchain protocols use digital signature algorithms, specifically Elliptic Curve Digital Signature Algorithm (ECDSA) to cryptographically sign transactions sent among peers. Public keys of the users published across all peers of the network and their integrity is protected through stored blocks. In blockchain protocols, transactions should have signatures that are specific to each transaction. If attacker does not have the private key of the original sender of the transaction, it is infeasible for her to generate valid signature, since validity of the signatures can be checked by public keys known by all peers. Therefore, proposed architecture does not allow tampering of transaction information between IoT devices.

\textbf{Block witholding} 
\cite{tamperingDelivery}
.
Tampering: In a Bitcoin network, after mining a block the miners broadcast the information about newly mined blocks. New transactions will be broadcast from time to time in the network. The network assumes that the messages will reach to the other nodes in the Bitcoin network with a good speed. However, authors in [64] ground this assumption, and they prove that the adversary can induce delays in the broadcast packets by introducing congestion in the network or making a victim node busy by sending requests to all its ports. Such type of tampering can become a root cause for other types of attacks in the network.
.
By slowing information propagation, attacker aims to generate inconsistency inside blockchain network. We discuss effects and how to defend system against such attack in Section \ref{sec:networkEclipse}.
.
 In performing \textbf{propagation delay attack}, attacker aims to generate inconsistency inside blockchain network by trying to make peers having different views of current state of the blockchain, in order to perform malicious activities.  
.
Propagation delay attack may also effect victim's view on current state of the blockchain, and may cause inconsistency to victim's operations.
.

\textbf{Transaction hiding:}








\subsection{Denial of service (DoS) attacks}
In general, DoS attacks may cause \textit{unavailability} of a subnet of IoT devices, by disrupting their resources and blocking valid requests and communication among devices. Proposed architecture can be  target of two types of DoS attacks as \textbf{DoS attacks targeting IoT devices} and secondly \textbf{DoS attacks targeting blockchain infrastructure}. 

%Buna gerek yok.
\textbf{DoS attacks targeting IoT devices} An attacker may perform DoS attack against IoT devices to interrupt correct execution of the IoT application and to capture the device. Moreover, effects of this attack to blockchain infrastructure depends on ratio of hashing power of victim devices to total hashing power of the blockchain network. If victim devices participate in private/consortium blockchain, such attack will not threat data integrity of blockchain, and new transactions generated by other devices can be executed correctly by remaining honest nodes. However, if honest target devices are participate in a public blockchain infrastructure, decrease of honest hashing power against rest of the nodes which might be malicious. In case malicious nodes become majority, they can perform 51\%attack that we discuss in the following Section \ref{sec:51attack}. We propose to use of strong authentication and authorization mechanisms on IoT devices an preventive mechanisms (e.g. \cite{ddosPreventiveIoT}, \cite{preventiveAdapDDoS}) against DoS attacks.   

\textbf{Dos attacks targeting blockchain infrastructure} An attacker may perform DoS attack against blockchain infrastructure using her malicious blockchain nodes in the network. 
Such attack is only effective against public blockchains, where anyone can participate in the network \footnote{We assume in private blockchains all peers are monitored closely by system administrators and if attacker compromise an IoT device and perform malicious activities, it can be detected easily and removed from the blockchain network}. 
Attacker may target to cause unavailability of system, by preventing processing of transactions honest peers, or attacker may try to keep honest peers busy with his transactions to waste their resources thus interrupt correct execution of the blockchain network. As such, this attack may cause double spend transactions to succeed, may generate delays on block and transaction propagation or may prevent valid transactions to be mined into the new blocks.
\subsubsection{DoS Attack Evaluation}\label{sec:dosEvaluation}
We have performed some Dos vectors targeting blockchain infrastructure by using Bitcoin protocol, and we have referred to Bitcoin stress test analysis in \cite{bitcoinStressTesting} for attack vectors. We have performed 4 different DoS attack vectors on emulated IoT devices that participate in Bitcoin network. In following, first we discuss our emulation settings then we present evaluated attacks and we discuss their their effects to the proposed architecture and how to protect against such attacks.

\subsubsection{DoS Attack Experimentation Structure}\label{sec:attackEmuStructure}
In our evaluations, we have emulated the victim IoT device using LXC system container tool. Emulated IoT devices run Ubuntu 16.04 (Xenial) operating system\footnote{releases.ubuntu.com/16.04/}. We have configured the victim IoT device with 512 MB of RAM and 50\% of one core of Intel Core i7 2.70 GHz CPU. We have used Bitcoin protocol's full node model for the victim IoT device, using bitcoind version 14.02. In order to attack emulated victim IoT device, we have emulated 10 attacker IoT devices using LXC system container tool, which run Alpine Linux operating system version 3.6.0. We set RAM limit of light peers to 128 MB, and limited CPU usage to 20\% of one core of Intel Core i7 2.70 GHz CPU. In order to perform DoS attacks on victim IoT device, we have developed attacker clients that run on attacker IoT devices. We have set Java SE, JRE 8 update 131 environment to our attacker IoT devices, and, we have developed attacker client applications with bitcoinj library using Java SE, JDK version 8 Update 131. All of our evaluations have been run on regtest network of Bitcoin protocol. 

\subsubsection{Sending many valid transactions} 
This DoS vector aims to overwhelm IoT device by increasing it's CPU usage, since peers of the blockchain networks have to check correctness of the transaction and if valid adding transaction to its memory. We have emulated the victim IoT device and 10 attacker IoT devices with configurations given in Section \ref{sec:attackEmuStructure}. In our experiments, attacker IoT devices continuously sent transactions directly to the victim device, the victim device has to check correctness of transactions and put into its memory if they are valid. We have performed to attack for 30 minutes, where in total 65000 transactions with one input (attacker node's account address) and one output address, sent to the victim device. We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:validTXs}, in which when attack started (around 15.01 in given figure) CPU usage increased significantly until attack has been terminated (around 15.31 in given figure). As such, 10 attacker IoT devices with previously given configurations, in average, managed to consume 35\% of the CPU power of the victim IoT device. Additionally, such attack generated 16 MB overhead to RAM usage of the victim IoT device.

\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Valid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with valid TXs}
  \label{fig:validTXs} 
\end{figure}
In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. In order to decrease possibility of successful attack, number of transactions that can be received from one peer in a period should be limited regrading resources of the IoT devices participating in the network. Additionally, this attack comes with its cost in Bitcoin network, since attacker needs to pay transaction fee for each transactions, therefore applying a transaction fee can also reduce chances for successful attack. 

\subsubsection{Sending many invalid transactions} 
This DoS vector aims to overwhelm victim IoT device increasing its CPU usage. As such, we have evaluated this attack vector on Bitcoin network by continuously sending invalid transactions with one input and one output addresses, from 10 emulated attacker IoT devices to the victim IoT device. Attacker IoT devices continued to attack to the victim IoT device around 20 minutes, where we continuously send may invalid transactions. We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:invalidTXs}, in which when attack started (around 09.50 in given figure) CPU usage increased significantly until attack has been terminated (around 10.10 in given figure). In given configurations with 10 attacker nodes, in average, attacker devices managed to consume 53\% of the CPU power of the victim IoT device.

\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Invalid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with invalid TXs}
  \label{fig:invalidTXs} 
\end{figure}

In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. In order to decrease possibility of successful attack, connection to the peer that send invalid transactions should be dropped. 


\subsubsection{Sending big transactions} 
This attack vector aims to overwhelm victim IoT device, since larger transactions including more operations requires IoT device's CPU and RAM usage. We have tested this attack vector by trying to send transactions from one attacker IoT device with increased transaction size, by adding many output addresses to the victim IoT device. As such, we have evaluated this attack vector on Bitcoin network by trying to generate and release big transactions, that we generate with an Bitcoin application developed using bitcoinj library.  We present our results by showing number of outputs that we put in single transaction, size of the transaction and whether generated transaction could be released into the network  in Table \ref{tab:bigTX}.
\begin{table}[t]
\centering
\caption{Sending Big Transactions}
\begin{tabular}{lllllll}
\hline
No of Output         & \multicolumn{1}{c}{100}  & \multicolumn{1}{c}{250}  & \multicolumn{1}{c}{500}  & \multicolumn{1}{c}{1000}  & \multicolumn{1}{c}{2930}  & \multicolumn{1}{c}{3000}  \\  \hline
TX Size                & \multicolumn{1}{c}{1 KB}    & \multicolumn{1}{c}{10 KB}   & \multicolumn{1}{c}{25 KB}   & \multicolumn{1}{c}{50 KB}   & \multicolumn{1}{c}{99 KB}   & \multicolumn{1}{c}{110 KB}  \\ \hline
Success         & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\textbf{X}}    \\ %\hline
\end{tabular}
\end{table}\label{tab:bigTX} 

As our findings verify, Bitcoin protocol limits maximum size the normal transactions as 100 KB. This attack may increase memory usage of IoT devices on the network, which may drop IoT devices from blockchain network by causing DoS. To decrease success possibility of this attack, maximum size of the transactions should be limited with regards to memory resource constraints of IoT devices on the network.


\subsubsection{Sending many big transactions} 
This attack aims to cause memory overwhelm of victim IoT device, by sending many transactions that each are generating many outputs. We have tested this attack vector by  sending as many transactions as possible from one attacker IoT device with many output addresses to the victim IoT device on Bitcoin network which is configured with the settings given in Section \ref{sec:attackEmuStructure}. In our experiments, we have varied transaction sizes by varying number of output addresses in transactions. We present our results by showing number of outputs that we put in each transaction, size of the transaction, how many transactions with given settings could be sent to the peer and size of the total overhead on memory of the IoT device in Table \ref{tab:manyBigTX}. Bitcoin protocol drops the connection to the attacker node after receiving certain amount of transactions, which we executed many times every attack and presented the average number.
 
\begin{table}[t]
\centering
\caption{Generating Big Transactions}
\begin{tabular}{lllllll}
\hline
No of Output         & \multicolumn{1}{c}{100}  & \multicolumn{1}{c}{250}  & \multicolumn{1}{c}{500}  & \multicolumn{1}{c}{1000}  & \multicolumn{1}{c}{2000}  & \multicolumn{1}{c}{2950}  \\  \hline
TX Size (KB)             & \multicolumn{1}{c}{3.6}    & \multicolumn{1}{c}{8.7}   & \multicolumn{1}{c}{17.1}   & \multicolumn{1}{c}{34.2}   & \multicolumn{1}{c}{68.2}   & \multicolumn{1}{c}{98.8}    \\ \hline
No of TXs        & \multicolumn{1}{c}{296}  & \multicolumn{1}{c}{193}  & \multicolumn{1}{c}{108}  & \multicolumn{1}{c}{63}  & \multicolumn{1}{c}{32}  & \multicolumn{1}{c}{22}  \\  \hline
Total Size (MB)     & \multicolumn{1}{c}{1.06}  & \multicolumn{1}{c}{1.67}  & \multicolumn{1}{c}{1.86}  & \multicolumn{1}{c}{2.15}  & \multicolumn{1}{c}{2.18}  & \multicolumn{1}{c}{2.17}  \\  \hline
\end{tabular}
\end{table}\label{tab:manyBigTX}    
    

This attack may increase memory usage of IoT devices on the network, which may drop IoT devices from blockchain network by causing DoS. Therefore, in order to decrease success possibility of this attack vector, firstly maximum size of the transactions should be limited with regards to memory resource constraints of IoT devices on the network. Secondly, total size of the transactions that can be received from a peer should be limited, and connection to the peer should be dropped by victim peer device.











INTRODUCTION

\iffalse
Traceability: BPIIoT platform can be used for developing traceability applications
for manufactured products. Smart contracts between the consumers and manufac-
turers can keep production records, for example, which factory and which machines
within the factory were used for manufacturing a particular product.
 Supply Chain Tracking: BPIIoT platform can be used for developing supply chain
tracking applications. The Blockchain and Smart Contracts can keep a formal regi-
stry of products and track their possession through different points in a supply
chain. Such applications can also enable automated financial settlements on delivery
confirmations.
Product Certification: BPIIoT platform can be used for developing product certifi-
cation applications. The manufacturing information for a product (such as the ma-
nufacturing facility details, machine details, manufacturing date and parts informa-
tion) can be recorded on the Blockchain. This information can help in proving the
authenticity of the products eliminating the need for physical certificates which can
be prone to tampering and forging.
 Consumer-to-Machine & Machine-to-Machine Transactions: BPIIoT can enable
machine-to-machine transactions for manufacturing services. For example, a con-
sumer can send a request for manufacturing a product by sending a transaction to a
manufacturer's smart contract along with the payment made in a crypto currency
(such as Ethers). The manufacturer’s smart contract can then send transactions to
smart contracts associated with individual machines (consumer-to-machine trans-
actions). If services of different machines are required for manufacturing a product,
the machines can send micro-transactions to other machines (machine-to-machine
transactions).
Tracking Supplier Identity & Reputation: BPIIoT platform can be used for devel-
oping supplier identity and reputation management applications which track vari-
ous performance parameters (such as delivery times, customer reviews and seller
ratings) for sellers. Such applications can be used by consumers to find the sellers
that can meet their manufacturing requirements and by manufacturers for finding
suppliers for consumables. Smart contracts can also help in automatically negotiat-
ing best prices for consumables and supplies in real-time based on the seller reputa-
tions.
Registry of Assets & Inventory: BPIIoT platform can be used for developing ap-
plications for maintaining records of manufacturing assets and inventory. These ap-
plications can keep records of the asset identification information and the transfer
of assets through the supply chain eliminating the need for manual paper records.
On-Demand Manufacturing: The BPIIoT platform will enable a marketplace of
manufacturing services where the machines will have their own Blockchain ac-
counts and the users will be able to provision and transact with the machines di-
rectly to avail manufacturing services in a CBM-like on-demand model. BPIIoT can
enable peer-to-peer networked manufacturing applications where the peers will be
able to avail manufacturing services (such as CNC machining or 3D printing) by
sending transactions to the machines.
Smart Diagnostics & Machine Maintenance: BPIIoT platform can be used for de-
veloping smart diagnostics and self-service applications for machines where the
machines will be able to monitor their state, diagnose problems, and autonomously
place service, consumables replenishment, or part replacement requests to the ma-
chine maintenance vendors. Smart contracts between manufacturers and vendors
for procurement of supplies and service of machines can help in automating the
machine maintenance tasks. We describe the implementation of a smart diagnostics
and machine maintenance application using the proposed platform in Section-7.
\fi
\iffalse
In ADEPT project \cite{ibmadept} of IBM and Samsung, autonomous decentralized peer to peer telemetry platform, IBM aims to achieve scalable and secure IoT systems by using blockchain technology as backbone. The ADEPT architecture consists three peer architectures, where classification is done according to the capabilities of devices (i.e. computational power, memory etc.) namely \textit{light peer} \textit{standard peer} and \textit{peer exchange}. \textit{Light peer} devices are with low level capabilities where they would have no capabilities of storing blockchains, and would only have its own blockchain address and balance inside the device. \textit{Standard peer} devices are capable of holding blockchain information for a certain period of time, where it can retain part of blockchain that is related to it or additionally also be for other \textit{light peer} devices in its ecosystem. \textit{Peer exchange} are high end devices with strong computing and storage capabilities; and able to  store blockchain, host marketplaces, demand supply chains etc.
\fi
%as its happening quite frequently lately \footnote{mirai, etc.},
%Moreover, considering high heterogeneity of IoT devices \cite{Whitmore2014}, enabling them to cooperate and generating a smooth execution environment is not an easy task. 
%Key objectives of the project are: accomplishing foundational IoT process tasks without centralized control infrastructure; having   robust security for transaction processing, storage, transport; and providing privacy by design. 
%ADEPT has been implemented using three protocols: TeleHash for peer to peer messaging among IoT devices, BitTorrent for file sharing, and Ethereum for blockchain and smart contracts. 
%Key element of the blockchain technology is an append-only, distributed and replicated ledger, where every transaction is recorded, and  cryptography techniques are used to  ensure data integrity, after achieving consensus on current state of the blockchain among peers 
\iffalse
@misc{buterinblockchainprivacy,
 author = {Vitalik Buterin},
 title = {{Privacy on the Blockchain}},
 howpublished = "\url{https://blog.ethereum.org/2016/01/15/privacy-on-the-blockchain}",
 year = {2015}, 
 note = "[Online; accessed 10-December-2016]"
}  
\fi














\iffalse
\subsubsection{Fixed difficulty}\label{sec:eva3.1}
We have varied block generation intervals from 3 minutes to 12 seconds with direct proportion to the number of devices on fixed block generation difficulty.  
Evaluation settings have been presented in Table \ref{tab:noDeviceSettings} and experiment results  in Table \ref{tab:case3.1Neds}, \ref{tab:case3.1Europe} and \ref{tab:case3.1World}.
.
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		   &{\bf 9H}  	 		    &{\bf 12H}	   		    &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:noDeviceSettings}
\end{table}
.
.
In all cases, increasing number of devices cause longer block propagation delays, which in turn increase stale block generation rates and decrease transaction throughputs.
Shorter block generation intervals cause system to produce more blocks.
However, due to higher number of devices and longer block propagation delay, stale block generation rates increase.
%Netherlands setting can achieve 25.11 transaction throughput
.
%1. case Netherlands 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{29.96}     &\textbf{0}	   &\textbf{29.96}    &  {\bf 0\%}	    &\textbf{7.85}           &{\bf 44.17}      & {\bf 9.86}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{76.67}     &\textbf{1.33}	   &\textbf{75.34}	  &  {\bf 1.73\%}	 &\textbf{6.97}          &{\bf 88.9}       & {\bf 25.11}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{101.29}     &\textbf{2}	    &\textbf{99.29}	  &  {\bf 1.97\%}	  &\textbf{8.07}     &{\bf 134.51}& {\bf33.09 }\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{177.67}     &\textbf{20.59}	    &\textbf{157.08}	  &  {\bf 11.52\%}	  &\textbf{41.19}     &{\bf 1168.86}& {\bf 52.36}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{237.18}     &\textbf{32.90}	    &\textbf{204.28}	  &  {\bf 13.87\%}	  &\textbf{147.13}     &{\bf 3485.49}& {\bf 68.09}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{216.45}     &\textbf{39.39}	    &\textbf{177.06}	  &  {\bf 18.2\%}	  &\textbf{291.87}     &{\bf 5791.87}& {\bf 59.02}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{211.98}     &\textbf{47.55}	    &\textbf{164.43}	  &  {\bf 22.43\%}	  &\textbf{498.97}     &{\bf 8265.55}& {\bf 54.81}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: Netherlands setting} \label{tab:case3.1Neds}
\end{table}
%2. case Europe 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{36.8}     &\textbf{0}	    &\textbf{36.8}	  &  {\bf 0\%}	  &\textbf{9.57}     &{\bf 44.6}& {\bf 12.26}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{62.49}     &\textbf{2.99}	    &\textbf{59.5}	  &  {\bf 4.78\%}	  &\textbf{8.91}     &{\bf 90}& {\bf 19.63}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{100.12}     &\textbf{5.2}	    &\textbf{94.92}	  &  {\bf 5.19\%}	  &\textbf{10.01}     &{\bf 138.76}& {\bf 31.64}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{176.55}     &\textbf{21.29}	    &\textbf{155.26}  &  {\bf 12.05\%}	  &\textbf{38.03}     &{\bf 1051.63}& {\bf 51.75}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{227.01}     &\textbf{46.61}	    &\textbf{180.4}	  &  {\bf 20.53\%}	  &\textbf{201.8}     &{\bf 3755.05}& {\bf 60.1}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{212.1}     &\textbf{49.51}	    &\textbf{172.59}	  &  {\bf 23.34\%}	  &\textbf{331.54}     &{\bf 6125.58}& {\bf 57.53}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{212.19}     &\textbf{55.08}	    &\textbf{157.11}	  &  {\bf 25.95\%}	  &\textbf{558.93}     &{\bf .}& {\bf 52.37}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: Europe setting} \label{tab:case3.1Europe}
\end{table}
%3. case World 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{32}     &\textbf{0.65}	    &\textbf{31.35}	  &  {\bf 2.03\%}	  &\textbf{10.13}     &{\bf 45.45}& {\bf 10.45}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{58.74}     &\textbf{3.62}	    &\textbf{55.12}	  &  {\bf 6.1\%}	  &\textbf{10.22}     &{\bf 91.27}& {\bf 18.37}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{98.29}     &\textbf{9.13}	    &\textbf{89.16}	  &  {\bf 9.28\%}	  &\textbf{13.01}     &{\bf 142.90}& {\bf 29.72}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{174.87}     &\textbf{28.17}	    &\textbf{146.7}	  &  {\bf 16.1\%}	  &\textbf{40.99}     &{\bf 1025.21}& {\bf 48.9}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{215.84}     &\textbf{43.7}	    &\textbf{172.14}	  &  {\bf 20.24\%}	  &\textbf{190.05}     &{\bf 3794.63}& {\bf 57.38}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{209.55}     &\textbf{50.62}	    &\textbf{158.93}	  &  {\bf 24.15\%}	  &\textbf{369.25}     &{\bf 6555.25}& {\bf 52.44}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{198.88}     &\textbf{57.12}	    &\textbf{141.66}	  &  {\bf 28.72\%}	  &\textbf{574.35}     &{\bf 11284.13}& {\bf 47.22}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: World setting} \label{tab:case3.1World}
\end{table}
.
.
.
.
.
\subsubsection{Varying difficulty}\label{sec:eva3.2}
We have varied number of IoT devices on fixed 1 minute block generation interval setting.
In which, difficulty of the PoW puzzle has been varied according to number of miners in the blockchain.
Evaluation results have been presented  in Table \ref{tab:case3.2Neds}, \ref{tab:case3.2Europe} and \ref{tab:case3.2World}.
.
In all evaluation cases, increasing number of devices cause to increase in block propagation delays, as every device have to check and propagate generated blocks.
In parallel,  stale block generation rates and lower transaction throughputs have been observed.
Netherlands case has the lowest stale block generation rates, due to low network latency.
In which, Netherlands setting complies with the integration metrics with up to 250 peers with given settings, whereas World setting does not comply with the metrics for any case due to high stale block rates. 
%1. case Netherlands 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  & \textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}        & \textbf{96.13}    &\textbf{0}       &\textbf{96.13}	    &  {\bf 0\%}	  &\textbf{9.38}          &{\bf 135.76}        & {\bf 32.04}\\
         \hline
         \textbf{12/166}    & \textbf{97.29}    &\textbf{0.33}	   &\textbf{96.96}	  &  {\bf 0.33\%}	 &\textbf{7.07}           &{\bf 133.37}       & {\bf 32.32}\\
         \hline         
         \textbf{18/250}    & \textbf{99.32}    &\textbf{1.78}	   &\textbf{96.65}	  &  {\bf 1.79\%}	 &\textbf{10.07}           &{\bf 136.37}       & {\bf 32.21}\\
         \hline 
         \textbf{36/500}    & \textbf{103.03}    &\textbf{4.42}	   &\textbf{98.61}	  &  {\bf 4.29\%}	 &\textbf{19.41}        &{\bf 122.99}       & {\bf 32.86}\\
         \hline  
         \textbf{54/750}    & \textbf{93.41}    &\textbf{4.49}	   &\textbf{88.92}	  &  {\bf 4.8\%}	 &\textbf{13.61}        &{\bf 102.03}       & {\bf 26.97}\\
         \hline 
         \textbf{72/1000}   & \textbf{93.03}    &\textbf{3.42}	   &\textbf{89.61}	  &  {\bf 3.67\%}	 &\textbf{19.41}        &{\bf 122.99}       & {\bf 32.86}\\
         \hline 
         \textbf{90/1250}   & \textbf{92.77}    &\textbf{2.98}	   &\textbf{89.78}	  &  {\bf 3.21\%}	 &\textbf{15.67}        &{\bf 107.01}       & {\bf 29.92}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: Netherlands setting} \label{tab:case3.2Neds}
\end{table}
%2. case Europe 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  &\textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}       & \textbf{105.97}    &\textbf{0.94}     &\textbf{105.93}	&  {\bf 0.88\%}	  &\textbf{12.88}        &{\bf 147.79}       & {\bf 35.31}\\
         \hline
         \textbf{12/166}     & \textbf{84.01}    &\textbf{1.64}	     &\textbf{82.37}	&  {\bf 1.95\%}	 &\textbf{8.40}          &{\bf 135.58}       & {\bf 27.45}\\
         \hline         
         \textbf{18/250}     & \textbf{100.03}   &\textbf{8.15}	     &\textbf{91.88}	&  {\bf 8.14\%}	 &\textbf{12.05}         &{\bf 146.13}       & {\bf 30.62}\\
         \hline 
         \textbf{36/500}     & \textbf{104.14}   &\textbf{7.89}	    &\textbf{96.25}	    &  {\bf 7.57\%}	 &\textbf{15.39}         &{\bf 148.11}       & {\bf 32.08}\\
         \hline  
         \textbf{54/750}     & \textbf{90.05}    &\textbf{6.38}	   &\textbf{83.77}	    &  {\bf 7.08\%}	 &\textbf{20.46}         &{\bf 168.43}       & {\bf 27.92}\\
         \hline 
         \textbf{72/1000}    & \textbf{97.44}    &\textbf{8.74}     &\textbf{88.70}	    &  {\bf 8.96\%} &\textbf{19.71}         &{\bf 155.68}       & {\bf 28.90}\\
         \hline 
         \textbf{90/1250}    & \textbf{82.78}    &\textbf{5.99}	   &\textbf{76.79}	    &  {\bf 7.23\%}	 &\textbf{18.43}        &{\bf 138.83}       & {\bf 25.59}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: Europe setting} \label{tab:case3.2Europe}
\end{table}
%3. case World 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  & \textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}        & \textbf{94.52}    &\textbf{4.3}      &\textbf{90.22}	&  {\bf 4.54\%}	 &\textbf{12.48}        &{\bf 146.97}        & {\bf 30.73}\\
         \hline
         \textbf{12/166}    & \textbf{95.17}      &\textbf{8.24}	 &\textbf{86.93}	&  {\bf 8.65\%}	 &\textbf{11.91}        &{\bf 142.04}        & {\bf 28.97}\\
         \hline         
         \textbf{18/250}    & \textbf{92.88}      &\textbf{7.2}	     &\textbf{85.68}	&  {\bf 7.75\%}	 &\textbf{11}           &{\bf 138.45}        & {\bf 28.56}\\
         \hline 
         \textbf{36/500}    & \textbf{99.83}     &\textbf{10.96}	 &\textbf{88.87}	&  {\bf 10.97\%} &\textbf{17.72}        &{\bf 150.56}         & {\bf 29.62}\\
         \hline  
         \textbf{54/750}    & \textbf{90.18}     &\textbf{7.46}	     &\textbf{82.72}	&  {\bf 8.27\%}	 &\textbf{19.45}        &{\bf 137.48}       & {\bf 27.57}\\
         \hline 
         \textbf{72/1000}   & \textbf{92.28}    &\textbf{11.44}	   &\textbf{80.84}	  &  {\bf 12.39\%}	 &\textbf{18.38}        &{\bf 140.83}       & {\bf 26.94}\\
         \hline 
         \textbf{90/1250}   & \textbf{82.03}    &\textbf{10.86}	   &\textbf{71.17}	  &  {\bf 13.24\%}	 &\textbf{20.01}        &{\bf 139.55}       & {\bf 23.72}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: World setting} \label{tab:case3.2World}
\end{table}
\fi








\iffalse
\begin{table*}  
\centering
\setlength{\tabcolsep}{10pt}
\begin{tabular} {|ccc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Aspects} &  \textbf{Vectors} & \textbf{Metrics} \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2}  \cmidrule(lr){3-3} 
%\midrule
\textbf{\textit{Scalability}} 	    &$\diamond$ No of devices		     		         & $\ast$ Maximum no of IoT devices as blockchain peers \\
\textbf{}		   			  		&$\diamond$ Transaction throughput of the system    & $\ast$ Maximum transaction throughput of blockchain system\\
\hline
\textbf{\textit{Security}} 	        &$\diamond$ Total amount of work     & $\ast$ Maximum result of the genuine block multiplied by  \\
\textbf{}		    		        &put to the blockchain				 &  difficulty of the PoW puzzle to generate a block\\
\hline
\textbf{\textit{Consensus}} 	&$\diamond$ Block propagation   &$\ast$ $\displaystyle\frac{\mbox{mean block propagation delay}}{\mbox{block generation interval}}$ $\leq$ 1 \\
\hline
\textbf{\textit{Resource}} 		&$\diamond$ Memory, processor, storage consumption  & $\ast$ Minimum difficulty of the PoW puzzle\\
\textbf{\textit{Consumption}}		&$\diamond$ Bandwidth consumption             & $\ast$ Average network traffic of a device $\leq$ 500 Kbps \\
\hline
\textbf{\textit{Efficiency }} &$\diamond$ Waste of energy and resources	 & $\ast$ Stale block generation rate  $\approx$ 1\%\\
\bottomrule             
\end{tabular}
\caption{IoT - Blockchain Integration Metrics} \label{tab:metrics} 
\end{table*}
\fi


%Therefore maximum number of IoT devices should be peers of the blockchain and  maximum transaction throughput should be achieved in the blockchain system.
%This is a very important issue that affects blockchain systems.
%For example, today's popular blockchain system Bitcoin having scalability issues due to low transaction throughput\footnote{$wikipedia.org/wiki/Bitcoin_scalability_problem$}, which led part of Bitcoin community to fork the Bitcoin blockchain and generate another coin named Bitcoin Cash\footnote{$en.wikipedia.org/wiki/Bitcoin_Cash$}, to process more transactions.

%Building on these aspects, we further specified vectors of these aspects, such as scalability - number of devices and transaction throughput.
%Finally, we specified IoT- blockchain integration metrics by considering needs and capabilities of IoT domain, that are presented in the Table \ref{tab:metrics}.



%\textbf{Novelty and value of the proposed architecture}
%\begin{itemize}
%\item Exploits decentralization, security and accountability features of blockchain technology on IoT domain. 
%\item Proposes multiple blockchains rather than a unique blockchain to offer better scalability and performance.
%\item Decreases in storage, memory and CPU overhead given by blockchain protocol to the IoT device . 
%\end{itemize}






%\textbf{Example scenario} Let us discuss an example IoT use case scenario with multiple blockchain architecture.  
%As discussed in \cite{supplyChainNetwork}, the supply chain network structure consists of many member firms and complex links between these firms, associated to the generation of a product, output value. Today's supply-chain systems have native needs like sustainability, transparency, visibility and need of decentralized infrastructure make supply chain scenario are good use case for integration of IoT and blockchain technologies. As the supply chain networks continues to grow in complexity, both in terms of the levels in the supply chain and the number of linkages, it can easily become untraceable \cite{complexSupplyChain}. 
%By integration of blockchain technology, immutable, shared and distributed nature of blockchains and permanent digital records of transactions may solve traceability issue and offer better provenance\footnote{www.wired.co.uk/article/wired-retail-2015}. 
%Given this, with the help of IoT technology using blockchain technology as background, enterprises may improve operational processes and reduce costs and risks due to transparency, traceability and adaptability. 
%In such a scenario, IoT devices  generation, transfer and update of products will be triggered by transactions of blockchain nodes. 
%Let us consider a very complex supply chain network, involving many suppliers and products, that generations massive amount of transactions.  
%Such a system will require high throughput of transaction execution, which might be a problem for a system of IoT devices with restricted resources. 
%Increasing number of blockchains, thus decreasing devices participating to the blockchain network offers to have better throughput and lower network latency of the system. 


%As an example, Bitcoin uses \textit{Simplified Payment Verification (SPV)}\footnote{www.bitcoin.org/en/developer-guide\#simplified-payment-verification-spv} protocol for light clients, where SPV protocol allows thin clients only to download block headers rather than all blocks to verify that particular transaction is indeed part of the block. In section \ref{sec:performanceLight}, we have tested and discussed about performance of the light clients of Bitcoin protocol, and we have showed that such methodology significantly decreases amount of resources used by the blockchain protocol.
%for such problems by transaction throughput needed. We want to underline that, design of such system is application specific, and capabilities of IoT devices and transaction volume between subset of devices plays a crucial role for design.
%\cite{supplyChainNetwork}
%So, instead of designing a new blockchain from scratch, our suggestion is to develop distributed applications for the IoT on top of the Bitcoin or another secure and stable blockchain. This can be done by leveraging a layered architecture, like the one proposed in Blockstack [40]. In this solution, the additional functionalities of the application are defined in another layer on top of the blockchain. Moreover, the blockchain is hidden at the application level, so low- performance IoT devices are not required to compute the PoW. 
%Relations: We could make use of Smart Contracts to set the rules on how the devices relate (collaborate) with each other. This way no intermediary is needed when any internet connected device wants to buy information or hire services from any other device. Also this intelligent agents may be able to negotiate prices (and discover new providers) to function autonomously.
%Payments. Payments, micro-payments and nano-payments between machines. Even bartering services could be possible. Hours of service of a particular device could be exchange for information provided for another one. Micropayment channels and nanopayments could be really useful in this scenario.
%We presume that for successful integration of blockchain technology into the IoT domain and to have more scalable architectural model, it is needed to exploit a multiple blockchain approach.
%Clearly, we need a backbone multi blockchain framework for proposed architecture. In section \ref{sec:systems}, discussion about multi-chain framework Polkadot, and its mechanisms and stakeholders has been given. 
%Applying IoT technology can optimize and affect whole supply-chain management paradigm by enabling  many features.
%In supply-chain systems, products have very complex and global manufacturing.
%As an example, IoT devices may be used as tools of asset tracking, which gives companies a way to improve their logistics operations and supply chain. Similarly, IoT technology allows to inventory and fleet management.
%IoT devices that capture finely granular real-time data about product and environment characteristics as well as location and timestamps throughout the supply chain, will be a solution for lack of a digital footprint, and improve provenance \cite{kim2016towards}.
%complexity of interactions between upstream and downstream linkages.
%Therefore let us discuss briefly about light client concept used by today's popular blockchain systems Bitcoin and Ethereum, since their light client ideology has effected our data structure design. Let us present \textit{Light Client Protocol (LCP)\footnote{\label{note1}www.github.com/ethereum/wiki/wiki/Light-client-protocol}} of Ethereum and \textit{Simplified Payment Verification (SPV)}\footnote{www.bitcoin.org/en/developer-guide\#simplified-payment-verification-spv} protocol of Bitcoin.
% Presentation of Ethereum's light client methods 
%LCP of Ethereum allows users in low capacity environments to maintain high-security assurance of verifying transaction executions and learning states of accounts without maintaining fully-synchronised database of Ethereum blockchain. In general, light client can be considered as a client that downloads block headers by default, and verifies only a small portion of what needs to be verified (transaction, state etc.), using a distributed hash table as a database for trie nodes in place of its local hard drive. In order to check whether a transaction is processed, light clients asks for block number including the particular transaction aimed to be verified and \textit{merkle path} of the merkle patricia tree including transaction. 
% Presentation of Bitcoin's light client methods 
%SPV protocol of Bitcoin allows thin clients only to download block headers rather than all blocks to verify that particular transaction is indeed part of the block. In SPV, client verifies that difficulty is high enough and block heads connected correctly simply checking previous hashes of each block and to verify transaction is indeed that particular block, they connect to a full node containing synchronized copy of blockchain, to get list of transactions in merkle path of the transaction to be verified. 
%Let us assume that supply chain scenario of a product consists involvement of many different products generated by different firms, each of which has its own lifecycle, which may include process phases of multiple companies and stakeholders.
%Let us present the potenatial challenges that may arise while IoT and blockchain integra
%\textbf{Multiple blockchain system} We propose a general multi-blockchain architecture, which assumes different blockchain protocols are able to send transactions to each other securely without losing accountability. ere are different proposals on multi-blockchain systems in literature like \cite{polkadot, cosmos,ethereumMauve}. In Section \ref{sec:architecture}, we discuss our expectations from such multi blockchain framework. Even though such back-end system is not in the scope of this paper, let us discuss an example of such multi-blockchain system, namely Polkadot. 
% \footnote{In Section \ref{sec:background} we briefly discussed an example heterogeneous multi blockchain project Polkadot} abilities to cooperate with each other, 
%We would like to underline that, our aim is not proposing an architecture for a specific IoT application, we do not focus on device structure, services or communication layers etc., but rather we propose methodology for the best integration of blockchain technology into IoT domain.
%The main motivation of the proposed architecture is providing 
%We assume blockchains used in proposed architecture will be able to communicate, and share transactions with each other.
%The proposed architectural model adjusts blockchain technology as a backbone technology, 
%\textbf{Architecture design principle}  
%Proposed architecture exploits foundational properties blockchain technology to build more robust and secure IoT systems, as discussed in Section \ref{sec:motivation}. In designing proposed architecture to generate a flexible architecture for IoT, we have considered diversity of the IoT ecosystem (e.g. device capabilities, application scenarios). Indeed, having common assumptions about IoT devices and application scenarios, and generating one size fits all design is not realistic for IoT domain. Therefore, we strongly believe that from architectural perspective being as general as possible is a must and protocol specifications of blockchains, like consensus protocols, should not be defined under strict terms. As an example, if we consider blockchain consensus protocols, there are always trade-offs between different protocols as discussed in \cite{quest}, and there is no optimal consensus solution that is best for every use case. As such, our core design principle is based on in this motivation. 
%-- IoT is mentioned as a possible field in which each device is identified by a public key to interact with other devices through the blockchain.
%Let us briefly discuss main features and what we expect from such multi blockchain back-end framework to be used as backbone framework for proposed multi  blockchain architecture. 
%Foremost important objective of such framework is processing inter-blockchain transactions with proved correctness and guaranteed overall system integrity in a secure way. 
%Firstly inter-chain transaction should at blockchain it is originated. If a transaction is not valid in its local blockchain, then the multiple blockchain framework should not accept it in the first place. 
%We presume, most likely such multiple blockchain framework will have its own blockchain to enhance security and integrity of the overall system.  
%Secondly, in order to have overall system integrity, a copy of each inter-chain transaction must be kept by the multiple blockchain framework, presumably in its blockchain, and integrity of the such transactions has to be ensured. 
%Finally, sending transactions from one blockchain to another have to be performed 
%There are different proposals on multi-blockchain systems in literature like \cite{polkadot, cosmos, ethereumMauve}. 
%\textbf{Connection of blockchains} Multiple blockchains will be able to send transactions to each other via inter-chain transactions, which will enable system to cooperate as like unique blockchain with increased interoperability.
%By exploiting inter-chain transactions, different application scenarios using their own local blockchain can cooperate with each other, without compromising accountability provided by blockchain technology.
%By recording inter-chain transactions, most likely in multiple blockchain framework's own blockchain, a process involving many participants from different blockchains will have accountability.
%may generate bottleneck for the system if they fully participate in blockchain protocols like consensus and block generation. 
%Proposed architecture aims to be suitable of complex systems including many heterogeneous IoT devices. 
%As such, for IoT devices with low capabilities, we propose to use of different roles of blockchain peers, as \textit{full peers} and \textit{thin clients} similar to Bitcoin\footnote{www.en.bitcoin.it/wiki/Clients}.
%There are two main scalability issues. The first is that, when the number of transactions grows, the blockchain increases in size, and it becomes expensive to store it, especially for IoT devices with limited resources.
%The second issue is the low throughput of transactions - a typical issue of the Bitcoin blockchain, which we did not find in the papers but is largely discussed within the Bitcoin community.



%(Even though, participants of the public blockchains can form up groups to take action together, such as mining pools of Bitcoin and Ethereum, which in some sense, may decrease the overall decentralization of the blockchain system).
%Another option is adoption to the existing public blockchains, such as Bitcoin or Ethereum.
%However adoption to the existing public blockchains is also not feasible, due to transaction fees and scalability issues considering number of devices and their capabilities..

%Such devices should be given with easier roles to perform like generating and sending transactions or checking block headers.
%However, they should not participate in the complex tasks such as block generation and consensus processes.

%Even though bigger blocks cause higher stale block generation rates, transaction throughput increases as they include more transactions.
%For example, in 1 minute block generation interval setting, with 100 KB blocks transaction throughput per second is 6.6 whereas with 10 MB block size, transaction throughput is 197.53, which is the highest transaction throughput we have observed in our evaluations.
%Moreover, long block propagation delays implies longer time to achieve consensus on the longest blockchain. 
%In our evaluations, we have observed observe this by comparing number of genuine blocks that have been generated in our evaluations in fixed time interval of 100 minutes.
%For example in 1 minute block generation interval setting, with 100 KB block size stale block rate is 0\% and number of genuine blocks is 99, whereas with 10 MB block size stale block rate is 35.07\% and number of genuine blocks is 26.93. 
%However, we have to note that, in case of higher network latencies and lower bandwidth capabilities, stale block rates will be higher.
%In such a case, bigger blocks will not imply higher transaction throughputs.
% Block generation interval: Block propagation time:  STALE RATES / Throughput  
%Similar to block sizes, also block generation intervals impact block propagation times, stale block rates, time required to achieve consensus and throughput.
%In IoT devices have to check and propagate blocks faster with shorter block generation intervals.
%However as IoT devices have limited resources and bandwidth capabilities, they may fail to finish block checking and propagation in short time intervals.   
%Indeed, this causes increase in the mean block propagation delays, as new generated blocks wait longer to be propagated across the network between IoT devices.
%For example with 500 KB block size, mean block propagation delay in 10 second block generation interval setting is 314.08 seconds, whereas it is 6.89 seconds in 5 minutes block generation interval setting.
%As expected, this in turn increases stale block rates of the system.
%For example with 500 KB block size, in 5 minute block generation interval setting stale block rate is 0\%,  whereas for 5 seconds block generation interval setting it is 45.96\%.
%However, for very small block sizes, short block generation interval settings do not increase stale block rates.
%For example with 10 KB and 50 KB block sizes, stale block rates are always lower than 1\%.
%In which, we have observed that, block generation interval and block sizes are not independent from each other and they should be set with respect to their values.
%As such, for big block sizes (e.g. 5 MB, 10 MB), long block generation intervals (e.g. 5 minutes, 10 minutes) have to be selected. 
%Whereas, for shorter block generation intervals (e.g. 10 seconds, 5 seconds), smaller blocks have to be used in the system (e.g. 10 KB or 50 KB).
%To conclude, block generation intervals have to be long enough regarding bandwidth capabilities of the IoT devices and block sizes.
%For IoT settings, using very big blocks are not suitable (e.g. 5 MB, 10 MB), as systems that have been configured with big blocks have long mean block propagation delay and achieve consensus later. 
%Thus, they have high stale block block generation rates and low transaction throughputs.
%On the other hand, very short block generation interval settings (e.g. 5 seconds, 10 seconds) result with long block propagation delay, high stale block generation rates and thus low transaction throughputs.
%As stale blocks are not part of the blockchain, they are lost efforts and waster of devices' resources and energy.
%Particularly, as the Netherlands setting has the shortest network latencies among nodes, best transaction throughput of 110.44 transaction per second have been observed in the Netherlands setting. 
%Higher block generation frequencies (e.g. 10 seconds, 5 seconds) increases stale block rates, thus, transaction throughputs are lower.  
%Our main inference from our observations on experiment results is; decreasing network latency among nodes is highly beneficial for blockchain adoption to IoT domain. 
%Indeed, having less network latency among nodes results with lower stale blocks and thus better transaction throughputs and faster consensus. 
%Particularly, a miner IoT device may not be aware of a new block that has been mined and published by another device due to long block propagation delays.
%In such a case, a miner IoT device would continue to mine and publish a new block by building on his view of the blockchain. 
%If we assume majority of the devices are aware of the new block and have already updated their local blockchains, the block published by unaware miner will be a stale block.
%However, stale blocks means lost efforts of the devices, thus, we prefer to have less stale blocks in the blockchain systems.
%We have observed the same behavior in evaluations results, that is, evaluations with
%Therefore long block propagation delays increase stale block rate.
%This means, the Netherlands settings have the lowest stale block rates in all evaluation cases with different block generation intervals.
%Transaction throughput of the system depends on number of genuine blocks, in which, low stale block rates imply high transaction throughput.   
%Therefore, the Netherlands setting have the highest transaction throughputs in all evaluation cases.
%Another important aspect effected by longer block propagation delays is the time required to achieve consensus, as its take longer time for the majority of the devices to have the same view of the blockchain.
%We can observe this by comparing number of genuine blocks that have been generated in our evaluations, as it presents the number of blocks that majority of the devices have consensed on fixed time interval (i.e. 100 minutes).
%Indeed, in our evaluation results, the highest number of genuine blocks have been observed in the Netherlands settings, for every block generation interval case.
%For example, for the 10 seconds block generation interval case, number of genuine block generated in the Netherlands setting is 133.23, whereas for %Europe setting it is 97.40. and for World setting it is 83.58.
%To conclude, shorter network latencies between IoT devices led blockchain system to have consensus faster, have lower stale block rates and higher transaction throughput. 
\iffalse
\begin{table*}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}    &{\bf Total}   &{\bf Average }  & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{delay}&\textbf{Traffic} &\textbf{Traffic} & \\ 
        \hline
         \textbf{10 MB} 	 & {\bf 139.06} 		& \textbf{101.79} 		 &{\bf 37.27}  			  &  {\bf 73.19\%}	 & {\bf 2342.38s}   & \textbf{3252.38s}	 &{\bf 3252.38s}  & {\bf 248.46 TX/s}  \\
        \hline
         \textbf{5 MB}		 & {\bf 176.25}		    & \textbf{134.46}		 &{\bf 41.79}  			  &  {\bf 76.20\%} 	 & {\bf 2314.44s}   & \textbf{3028.62s}	 &{\bf 3252.38s}  & {\bf 139.30 TX/s}  \\
        \hline
         \textbf{1 MB}		 & {\bf 322.39} 		& \textbf{247.72} 		 &{\bf 74.67}     		  &  {\bf 76.83\%} 	 & {\bf 1752.36s}   & \textbf{2499.64s}  &{\bf 3252.38s} & {\bf 49.78 TX/s} \\
        \hline
         \textbf{500 KB} 	 & {\bf 426.35}         & \textbf{327.40} 	     &{\bf 98.95}             &  {\bf 76.79\%}   & {\bf 1596.04s}   & \textbf{2360.82s}  &{\bf 3252.38s}   & {\bf 32.98 TX/s}\\
        \hline
         \textbf{100 KB}     & {\bf ...}         &\textbf{}         &{\bf }             &  {\bf \%}   & {\bf s}   & \textbf{s}  &{\bf GB}   & {\bf TX/s} \\
        \hline 
         \textbf{50 KB} 	 & {\bf ...}         &\textbf{}         &{\bf }             &  {\bf \%}   & {\bf s}   & \textbf{s}  &{\bf GB}   & {\bf TX/s} \\
        \hline      
         \textbf{10 KB}       &{\bf 5361.31}        &\textbf{54.45}           &{\bf 5306.86}          &  {\bf 1.01\%}     & {\bf 3.00s}     & \textbf{0.49s}  &{\bf 3252.38s}   & {\bf 35.37 TX/s}  \\
        \hline    
    \end{tabular}
\caption{1 second block generation interval setting} \label{tab:1sec}
\end{table*}
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		  &{\bf 9H}  	 		  &{\bf 12H}	   		  &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:caseSettings}
\end{table}
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings}   & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Netherlands}& \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
         \hline
          \textbf{Europe}     & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		  &{\bf 9H}  	 		  &{\bf 12H}	   		  &{\bf 15H}   \\
       \hline
        \textbf{World}        &\textbf{3 mins}		 & {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:caseSettings}
\end{table}
\begin{figure} [H]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/chart2.png}
	\caption{ Cost - difficulty relation \label{fig:cost2}}
\end{figure}
\fi


\subsection{Req Findings}\ref{sec:reqFindings}
%Let us exploit the Bitcoin simulator presented in \ref{sec:simulatorSettings} to test transaction throughput of a proposed setting and unique blockchain setting, in fixed 500 Kb block size setting with regards to blockchain-IoT integration metrics presented in Section \ref{sec:metrics}.
%For example by having 250 IoT devices in \textit{the Netherlands} setting, the shortest block generation interval setting is 30 seconds and number of transactions per device in a minute is 12.
%However, as a unique blockchain setting by having 2000 IoT devices in \textit{World} setting, the shortest block generation interval setting that satisfies blockchain-IoT integration metrics given in Section \ref{sec:metrics} is 12 minutes and number of transactions per device in a minute is 0.1.
%In proposed setting, devices in different subgroups are able to send transactions to each other.
%Therefore, dividing IoT devices into subgroups do not cause to decrease number of devices participating in the system.
%In overall system, multiple blockchains contain same amount of devices a unique blockchain, with much lower stale block generations rates and block propagation delays (as evaluated in Section \ref{sec:reqEva1}, \ref{sec:reqEva2} and \ref{sec:reqEva3}).


%Several features of blockchain technology and characteristics of IoT domain should be taken into consideration to enable blockchain technology into the IoT domain.
%To evaluate and analyze such features, we specified a set of integration metrics that is presented in Section \ref{sec:metrics}.
%We have evaluated many features of blockchain IoT integration by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings} and referring to the blockchain IoT integration metrics.




PERFORMANCE

%We recall that in proposed architecture three roles have been defined for IoT devices as: outsider devices, light peer devices and full peer devices.
%Light and full peer devices directly peers of the blockchain network, thus blockchain operations affect their performance.
%However, outsider devices aren't peers of the blockchain and they do not perform blockchain operations, thus being part of a blockchain network doesn't affect their performance.
%Given that, we evaluate performance of the light peer and full peer devices.
%To measure and monitor performance of 

%In our DoS attack scenario, a full peer device is the victim device, and it is attacked by 10 (DoS scenario \rom{1}) and 20 (DoS scenario \rom{2}) light peer devices by sending many transactions.
%This DoS attack aims to overwhelm IoT device by increasing it's CPU usage and bandwidth consumption as it has to check correctness of each transaction.
%We generated two DoS scenarios as DoS scenario \rom{1} with 10 attacker devices and \rom{2} with 10 attacker devices.
%For both of evaluation cases we performed to attack for 45 minutes.
%In DoS scenario \rom{1} 83100 transactions sent by attacker devices with an average of 8100 transactions per attacker. 
%Whereas, in DoS scenario \rom{2} 108960 transactions sent by attacker devices with an average of 5448 transactions per attacker. 
%Decrease in number of transaction send by an attacker device decrease in DoS scenario \rom{2} due to overwhelm of the victim IoT device.




%where in total 65000 transactions with one input (attacker node's account address) and one output address, sent to the victim device. 
%Due limited resources of light peer devices, light peer devices run Alpine Linux operating system\footnote{alpinelinux.org} version 3.6.0, that is a lightweight Linux o.s. distribution that only requires around 5 MB of storage. 
%Whereas, light peer devices set up with 120 MB of RAM, and their CPU usage is limited to 2\% of one core of Intel Core i7 2.70 GHz CPU. 
%We have evaluated the effect of size of the blockchain to resource usage of IoT devices acting as full peers of blockchain network by using device configuration settings previously given in Section \ref{sec:emulationStructure}. 
%noktalar arasi direk 5.3 Eva 2 ye gitcek
%First, in order to test performance of the full peers and scalability of the proposed architecture, we have emulated 200 IoT devices on IBM Power 8 server. 
%IoT devices configured with 512 MB of RAM (memory swap is disabled) and 5\% of a single Power8 CPU\footnote{https://www-01.ibm.com/common/ssi/cgi-bin/ssialias?htmlfid=POB03046USEN}, which has 3.5 GHz clock rate. 
\iffalse
\begin{figure*} 
    \centering
  \subfloat[20 nodes]{%      
     \includegraphics[width=0.25\linewidth]{figures/CPU_Utilization-10lu.png}}
  	  \label{1a}\hfill
  \subfloat[40 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/CPU_Utilization-20li.png}}
    \label{1b}\hfill
  \subfloat[100 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1c}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1d} 
  \caption{(a), (b), (c), (d).}
  \label{fig:CpuUtil} 
\end{figure*}
\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
     \includegraphics[width=0.5\linewidth]{figures/CPU_Utilization-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/CPU_Utilization-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}

\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}



 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}
	\caption{Full peer ETH Sce \rom{1}} \label{fig:architecture}
\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/Total_Ethernet_Read_and_Write-20li.png}
	\caption{Full peer ETH Sce \rom{2}} \label{fig:architecture}
\end{figure}

 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/CPU_Utilization-10lu.png}
	\caption{Full peer 10lu} \label{fig:architecture}
\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/CPU_Utilization-20li.png}
	\caption{Full peer 20li} \label{fig:architecture}
\end{figure}


\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Lightcpu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Lighteth0.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}
\fi

\iffalse
% \begin{figure} [h] 
%	\centering
%	\includegraphics[height=50mm]{figures/Lighteth0.png}
%	\caption{Light peer ETH} \label{fig:architecture}
%\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[height=50mm]{figures/Lightcpu.png}
	\caption{Light peer CPU} \label{fig:architecture}
\end{figure}
\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}
\fi

\iffalse
  \subfloat[Full Peer  Network]{%
      \includegraphics[width=0.33\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[Full Peer Sce \rom{2} Network]{%
      \includegraphics[width=0.33\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
\fi


\iffalse
\begin{figure*} 
    \centering
  \subfloat[Light Peer CPU CPU]{%
      \includegraphics[width=0.33\linewidth]{figures/Lightcpu.png}}
     \label{c} 
  \subfloat[Full Peer Sce \rom{1} CPU]{%
     \includegraphics[width=0.33\linewidth]{figures/CPU_Utilization-10lu.png}}
     \label{b}\hfill
  \subfloat[Full Peer Sce \rom{1} CPU]{%
      \includegraphics[width=0.33\linewidth]{figures/CPU_Utilization-20li.png}}
     \label{c}      
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure*}
\fi





%Scalability is the biggest challenge to overcome in adapting blockchain technology into the IoT domain.
%Optimal blockchain system should have high transaction throughput and maximum number of nodes should participate in the blockchain.
%Therefore, we go for a hybrid blockchain architecture, both containing PoW and BFT blockchains, as a solution for scalability problem of IoT domain.
%Particularly, first IoT devices divide into subgroups and form PoW blockchains, like as sharding of a unique blockchain that would contain all devices.


%Sharding PoW blockchains requires elaborate evaluation of scalability, performance and security aspects have to be considered carefully. 
%We propose blockchain-IoT integration metrics to achieve high performance and scalability.
%If sharding a PoW blockchain into multiple blockchains decrease amount of work that each new blockchain contains, than they are more vulnerable against threats target their integrity.
%Given, that we quantitatively evaluated effects of sharding. 
%Therefore, we go for a hybrid blockchain architecture containing PoW and BFT blockchains. 
%Two popular blockchain consensus models, namely PoW and BFT, provide effective solutions to the different parts of the scalability problem \cite{quest}. 
%Particularly, PoW based blockchains are able to scale to thousands of nodes and BFT based blockchains can achieve thousands of transaction throughput.



\iffalse
Improving the performance of PoW blockchains. Sompolinski and Zohar GHOST (Greedy Heaviest-Observed Sub-Tree) rule [55], which
basically resolves conflicts in a PoW blockchain by weighing the subtrees rooted in blocks rather than the longest (sub)chain rooted in given blocks. 
Although
GHOST is essentially a conflict-resolution strategy, it offers performance benefits
over the standard longest (heaviest) chain rule of Bitcoin, as it provides more
secure means of increasing the block frequency and the block size [55]. A variant
of the GHOST rule is actually implemented in the Ethereum blockchain [58],
although the GHOST-PoW performance has not yet been adequately stresstested
with high loads (in 2016, typical Ethereum throughput is fewer than
20,000 transactions per day, i.e., about 0.2 tx/s on average).5
\fi


\iffalse
Hyperledger in yeni konsepti vukolic in paper dan
a. The new architecture [1], termed Fabric V1
here, separates the execution of smart-contract transactions (in the sense of validating the
inputs and outputs of a program) from ordering transactions for avoiding conflicts (in the
sense of an atomic broadcast that ensures consistency). This has several advantages, including
better scalability, a separation of trust assumptions for transaction validation and ordering,
support for non-deterministic smart contracts, partitioning of smart-contract code and data
across nodes, and using modular consensus implementations [59].
\fi
%In addition to performing inter-chain transactions, blockchain connector framework contains and executes smart contracts for all sub-blockchains, that are self-executable programs in the blockchain\cite{szabo}.
%The reason to separate smart contracts in spe
%Quest: Indeed, a smart contract can be modeled as a state machine, and its consistent execution across multiple nodes in a distributed environment can be achieved using state machine replication.
%BFT based multiple blockchain connector framework perform inter-chain and smart contract transactions of sub-blockchains and able to perform thousands of transactions per second \cite{consensusWild}.
%.

==> DEPRECATEDbackground.tex <==
\section{PoW Blockchains Background}\label{sec:background}
In this section, we provide a brief background information on PoW blockchains.
%Blockchain refers to distributed database, a shared ledger, on a peer to peer network. 
%Novelty of the blockchain technology lies in its ability to achieve coordination and verification of individual activities carried out by different parties without a centralized authority or trusted third party \cite{blockchainTechnology}.


\textbf{Blockchain structure.} 
Transactions transfer information (i.e. data packets) between peers and they have unique identifiers, input data, and they are bundled into data chunks called blocks. 
Every block contains set of transactions, a timestamp, a reference to the preceding block, and an authenticated data structure (i.e. a merkle tree) from previous transactions, and forms the blockchain. 
Blockchains are peer to peer networks, and nodes are connected to other nodes as peers to share transactions and blocks. 
A copy of the blockchain is stored on every node in the network and these peers exchange the latest block information with each other to ensure that all of them have the same shared database.


\textbf{PoW - block generation.}
Blockchain nodes have to solve a cryptographic puzzle, Proof of Work (PoW), to be authorized to generate a new block.
In generating a new block, miners nodes confirm that new transactions are valid and consistent with former transactions before sealing them into blocks. 
Main duty of the PoW is preventing instant block creations to reduce conflicts such as double spending and sybil attacks. 
Indeed, attackers can't easily create many blocks to shape an alternative blockchain, however it is easy to confirm once it is created.
Blockchain nodes trying to generate a new block is called \textit{miners}, block generation process is called \textit{mining}, miner's mining ability is referred as \textit{mining power}.
In PoW blockchain, difficulty of the PoW puzzle is used regulate expected average block generation interval according to the total mining power of the miners in the blockchain network.
In particular, to have a fixed block generation interval, difficulty is increased when total mining power increases, and it is decreased when total mining power decreases.


\textbf{Block sharing.}
Miners share the new found block with its peers at the time of solving the PoW puzzle.
Nodes that have received the new block are responsible for checking the correctness of the block, and legitimacy of the transactions inside the block, ensuring that they have not been included in any other block previously, before adding blocks to their local blockchain and propagating to their peers. 
Adding new blocks to the blockchain increases total amount that blockchain contains, and thus it increases security of the blockchain against adversaries trying to alter it.


\textbf{Stale blocks.}
Blockchains may have forks due to malicious manipulations or propagation delays and longest fork remains as the agreed and valid blockchain branch\cite{blockchainSurvey}(to the rest of the paper we will refer blocks included to the blockchain as genuine blocks). 
In general, blocks in shorter forks do not included in the blockchain and they referred as \textit{stale blocks}\footnote{In Ethereum blockchain(ethereum.org) they are included to the blockchain as uncle blocks, however they do not count towards total difficulty of the blockchain \cite{onTheSecurityPoW}}.
Stale blocks do not contribute to the security of the blockchain and transactions in stale blocks considered as unprocessed by the network, thus stale blocks should be considered as lost of efforts.
%In this case, the rate of discarded blocks (known as the orphan rate or the fork rate) increases and the security of the protocol deteriorates. 




Blockchains can be categorized into two groups with regards to their consensus methodologies as \textit{Proof of Work (PoW)} and \textit{Byzantine Fault Tolerant (BFT)} blockchains.
In PoW-based blockchains, such as Bitcoin \cite{bitcoinNakamoto} and Ethereum \cite{ethereumYellowpaper}, peers have to solve a cryptographic puzzle as proof of their work in order to be authorized to generate a new block. 
PoW-based blockchains able to scale thousands of nodes in achieving consensus. 
On the other hand BFT-based blockchain protocols, such as Hyperledger \cite{hyperledger}, achieve consensus by state replication with assumption of limited number of faulty peers.
BFT-based blockchain protocols can achieve thousands of transactions throughput \cite{quest}.




%This should be handled as a twofold issue; first one is the low hardware resources, and  second one is the limited available bandwidths.
%Due to low hardware resources, such as memory or processor, the PoW puzzle should be set as easy as possible, as devices should not devote all of their resource to generate a block.
%In which, amount of work to generate a block and number of  blocks that blockchain contains are two main factors that affect security of the blockchain.
%that is the total amount of mining process required to generate the whole blockchain.


%\cite{blockchainGraphprimer}
%Nodes converge to a single agreed version by selecting the chain containing the highest amount of computational work as the valid version (usually the longest chain). 
%The proof-of-work also serves to limit the ability of attackers to subvert the system: they cannot easily create many blocks, which would potentially allow them to create a longer alternative chain that will be adopted by nodes and thus reverse the transfer of funds (double spend).
%\textbf{Addresses}
%Address is a unique string of 26-35 characters created from public key.
%The source and destination addresses are represented by a cryptographic hash of a public key of the respective user.
%In case of Bitcoin, the private key of the user is required to spend coins in form of the digitally signed transactions.
%Stale tanimi : Conflicts, which take the form of blocks that extend the same parent, represent alternative sets of accepted transactions. 
%\textbf{Blockchain types:} Blockchains can be classified into three groups: \textit{public blockchains}, \textit{private blockchains} and \textit{hybrid(consortium) blockchains}\footnote{blog.ethereum.org/2015/08/07/on-public-and-private-blockchains/}. Public blockchains are open to the participation of anyone in the world, where anyone can read, send transactions, and participate in the consensus operation. Such blockchains offer full decentralization, e.g. Bitcoin\footnote{bitcoin.org} and Ethereum\footnote{ethereum.org}. In private blockchains, an organization holds permissions about who can write to the blockchain and take part in the consensus protocol and granting these rights are based on invitation. In consortium blockchains, a set of nodes are responsible from consensus operation, where similarly to the public blockchains reading permissions may be public or restricted.
%\textbf{How blockchain operates} Transaction validation depends upon to rules of the particular blockchain network's application logic. As an example, in Bitcoin, transaction must have enough total bitcoin in its inputs to cover the output. Every input of transaction must have right to spend the prior output to which it is connected and each output of a transaction can be spent once \footnote{www.en.bitcoin.it/wiki/$Protocol\_{rules}$}. More precisely, peers are incentivised to generate a block by rewards. As an example, today, in Bitcoin the peer generating a new block receives 12.5 bitcoins.
%IoT Security Problem
%Indeed, considering growth of the IoT market and new interconnected devices, increases attack surface since each of them can become the weakest link and exploited \cite{learningIoTsecurity}. As discussed in \cite{securingIoT}, benefits of IoT could easily be suspended and outweighed by security vulnerabilities of it. IoT is facing with serious security problems like identity management and encryption \cite{Whitmore2014}, access control and authentication \cite{sicariSecurity}.
%IoT interoperability problem
%To reach true potential of the IoT, sensed and processed data must be exchanged and analyzed with other applications in order to generate valuable information. Therefore things must be able to connect and access information provided by other things without compromising their security and privacy. As such, interoperability must be ensured in order to turn raw data into valuable and useful information. However, if we consider heterogeneity of IoT devices \cite{Whitmore2014}, achieving interoperability becomes challenging. 
%\textbf{Interoperability}: WILL CHANGE. 
%Decentralization of IoT is very beneficiary since it overcomes the problem of a single point of failure.Indeed, decentralization of IoT architectures is a must, considering increasing number of IoT devices and high infrastructure and maintenance costs. Therefore, IoT should shift from central architectures to \textit{decentralized architectures}. Massive number of IoT devices, expected to be around twenty billions according to ITU \cite{ituIoT}, is generating crucial \textit{scalability issue}. Additionally to being massive, if we consider heterogeneity of IoT devices (as discussed in \cite{Whitmore2014}), the \textit{interoperability} problem arises as a very important issue. 
%Blockchain foundational properties of blockchain, we claim that blockchain technology offers great opportunities for achieving decentralization, security of applications of various domains. 
%Polkadot achieves low-level consensus over a set of mutually agreed and valid block through asynchronous \textit{Byzantine Fault Tolerant (BFT)} algorithm.
%Polkadot network consists four basic roles to keep up the network, namely \textit{Validator}, \textit{Nominator}, \textit{Collator} and \textit{Fisherman}. 
%In summary, validator helps seal new block on the Polkadot network, which refers to relay chain and all parachains.
%A Validator must run a relay-chain implementation with high availability and bandwidth, in order to be ready to accept new block on a nominated parachain. 
%Validator receives the block from nominated parachain, validates it, and then republishes the block. 
%Validation of a block requires fully-synchronized database of the parachain, but since maintaining all of the parachains is not reasonable, validator will nominate the task of devising a suggested new parachain block to collator. 
%Collator assists validator in producing valid parachain blocks. 
%Collators maintain a "full-node" in particular parachain, meaning that they can retain all information required to author new blocks and execute transactions. 
%Nominator is a stake-holding party contributing security bond of a validator. 
%Nominators select validators that they trust to act responsibly in maintenance of the network, and they place risk capital to such validator.  
%Fishermen are independent "bounty-hunters", they get their reward by proving one bonded party acted illegally.

==> DEPRECATEDrelated.tex <==
\section{Related Work}\label{sec:related}

In literature there are different proposals proposing use of blockchain technology. In \cite{blockchainIIOT}, a blockchain platform for industrial IoT (BPIIoT) has been proposed, which enables development of decentralized manufacturing applications of cloud based manufacturing. IoT devices run blockchain services and contain blockchains wallets for sending transactions to the smart contracts of blockchain service, and connection to the cloud and drivers for the sensors to push sensor data into the cloud. Proposed blockchain platform make use of blockchain technology to execute smart contracts, which does not exploit main features of blockchain technology to secure IoT applications. 
In \cite{optimizedBLCIOT}, a blockchain architecture for IoT proposed, which aims to decrease overhead of blockchain protocols given to IoT devices. Proposed architecture exploits immutable ledgers that are managed centrally with local devices, where transaction requests send to a peer of public blockchain network, where for subset of peers elects a Cluster Head (CH) that is participating in public blockchain. Authors tried to decrease of network overhead by using trust table, with decreasing amount of transactions to be verified sent by CH if it has high trust. However, by node compromise attack on CH device,  malicious transactions may be sent, without much verification. Additionally, many devices from many device subsets send transactions to the public blockchain, which does not solve main scalability issue of having high number of IoT devices generating massive amount of transactions.
Differently from previous works, the Tangle \footnote{$iota.org/IOTA_Whitepaper.pdf$} protocol implements a global distributed ledger by using Directed Acyclic Graph (DAG) generated by transactions, as a blockchainless approach. The tangle  designed as a cryptocurrency for the Internet of Things by aiming to make micro-payments possible, where every new transaction has to approve two previous transactions to be included in the DAG.  

==> DEPRECATEDsecurity.tex <==
%ESKI.
%girizgah tamam. sonuclar ve yorumlari yok.
\subsubsection{Security Evaluation \rom{1} - Fixed difficulty}\label{sec:secEva1}
We have evaluated how varying number of devices on the fixed difficulty of the PoW puzzle affect security of the blockchain.
Experiment cases have been taken from Table \ref{tab:caseSettings},
In which, block generation difficulty is fixed and total hash rates of devices have been simulated by varying block generation intervals with regards to number of devices.
IoT devices locations have been simulated using three location settings as; The Netherlands, Europe and World location settings presented in Section \ref{sec:settings}.
Moreover, in all cases, we have assumed every device has the same mining power and we have fixed block size to 500 KB.
Evaluation results have been presented in Table \ref{tab:secEva1Neds}, \ref{tab:secEva1Europe} and \ref{tab:secEva1World}.



As presented in evaluation \rom{2} at Section \ref{sec:eva2}, block sizes can distinctively affect the blockchain network, and best block size  settings for IoT is in range of 100 KB to 1 MB.
Thus, for the sake of our evaluations, we have fixed block sizes to 500 KB.






\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Total Blocks}       & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{in}                 & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Forks}	         & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{29.96}     &\textbf{0}	   &\textbf{29.96}    &  {\bf 0\%}	    &\textbf{0.85}           &{\bf 44.17}      & {\bf 9.86}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{55.78}     &\textbf{3.49}	   &\textbf{52.29}	  &  {\bf 6.25\%}	  &\textbf{1.06}       &{\bf 181.01}     & {\bf 34.86}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{99.08}     &\textbf{7.6}	    &\textbf{91.48}	  &  {\bf 7.67\%}	  &\textbf{2.91}     &{\bf 493.68}& {\bf 60.98}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{147.13}    &\textbf{25.44}	&\textbf{121.69}  &{\bf 17.29\%}      &\textbf{13.64}    &{\bf 4299.61}& {\bf 81.12}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{153.99}    &\textbf{35.47}	&\textbf{118.52}  &  {\bf 23.03\%}  &\textbf{26.3}        &{\bf 7736.09}& {\bf 79.01}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{145.79}    &\textbf{42}		&\textbf{103.79}  &  {\bf 28.80\%}  &\textbf{36.87}    &{\bf 11809.46}& {\bf 69.19}\\
         \hline 
         \textbf{Case \rom{7}} 	& \textbf{134.32}    &\textbf{38.44}	&\textbf{95.88}	  &  {\bf 28.61\%}  &\textbf{47.60}    &{\bf 16518.03}& {\bf 63.92}\\
         \hline       
    \end{tabular}
\caption{Security evaluation \rom{1}: Netherlands setting} \label{tab:secEva1Neds}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Total Blocks}       & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{in}                 & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Forks}	             & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{31.55}     &\textbf{0.33}	    &\textbf{31.22}	   &  {\bf 1.04\%}	 &\textbf{1.59}         & {\bf 20.81}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{60.08}     &\textbf{4.32}		&\textbf{55.76}	   &  {\bf 7.19\%}	 &\textbf{2.9}          & {\bf 37.17}\\
         \hline
         \textbf{Case \rom{3}}   & \textbf{86.09}    &\textbf{5.9}		&\textbf{80.19}	   &  {\bf 6.85\%}	 &\textbf{4.94}         & {\bf 53.46}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{143.09}    &\textbf{29.34}	&\textbf{113.75}   &  {\bf 20.54\%}	 &\textbf{10.84}        & {\bf 75.83}\\
         \hline 
         \textbf{Case \rom{5}}   & \textbf{139.46}   &\textbf{33.32}	&\textbf{106.14}   &  {\bf 23.89\%}  &\textbf{25.22}        & {\bf 70.76}\\
         \hline 
         \textbf{Case \rom{6}}   & \textbf{135.28}   &\textbf{37.87}	&\textbf{97.41}	   &  {\bf 27.99\%}  &\textbf{37.69}        & {\bf 64.94}\\
         \hline 
         \textbf{Case \rom{7}}   & \textbf{138.05}   &\textbf{42.18}	&\textbf{95.87}	   &  {\bf 30.55\%}  &\textbf{68.56}        & {\bf 63.91}\\
         \hline       
    \end{tabular}
\caption{Security evaluation \rom{1}: Europe setting} \label{tab:secEva1Europe}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Total Blocks}       & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{in}                 & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Forks}	             & \\
         \hline
         \textbf{Case \rom{1}}    & \textbf{31.16}    &\textbf{0.33}   &\textbf{30.83}	  &  {\bf 1.05\%}	 &\textbf{17.99}             & {\bf 20.55}\\
         \hline
         \textbf{Case \rom{2}}    & \textbf{73.7}    &\textbf{7.09}	   &\textbf{64.61}	  &  {\bf 9.62\%}	 &\textbf{34.65}             & {\bf 43.07}\\
         \hline         
         \textbf{Case \rom{3}}     & \textbf{87.05}    &\textbf{12.3}    &\textbf{74.75}    &  {\bf 14.12\%}  &\textbf{47.73}            & {\bf 49.83}\\
         \hline 
         \textbf{Case \rom{4}}     & \textbf{146.45}   &\textbf{28.85}	 &\textbf{117.6}	&  {\bf 19.69\%}  &\textbf{53.61}           & {\bf 78.40}\\
         \hline  
         \textbf{Case \rom{5}}     & \textbf{141.59}   &\textbf{35.29}	 &\textbf{106.3}    &  {\bf 24.92\%}  &\textbf{70.68}           & {\bf 70.86}\\
         \hline 
         \textbf{Case \rom{6}}     & \textbf{139.32}   &\textbf{42.23}	 &\textbf{97.09}	&  {\bf 30.31\%}  &\textbf{80.77}           & {\bf 64.72}\\
         \hline 
         \textbf{Case \rom{7}}    & \textbf{140.56}    &\textbf{48.3}	 &\textbf{92.26}	&  {\bf 34.36\%}  &\textbf{98.99}           & {\bf 61.50}\\
         \hline       
    \end{tabular}
\caption{Security evaluation \rom{1}: World setting} \label{tab:secEva1World}
\end{table}








%YENI
%girizgah tamam. yorum ve sonuclar yok.
\subsubsection{Security Evaluation \rom{2}: varying difficulty, fixed Block generation interval}\label{sec:secEva2}
We have evaluated how varying difficulty of the PoW puzzle according to number of nodes on different location settings effects security of the blockchain. 
Number of IoT devices has been varied as 83, 166, 250, 500, 750 and 1000, in which, 6, 12, 18, 36, 54 and 72 have been given with the miner role, respectively.
We have assumed every device has the same mining power.
Difficulty of the PoW puzzle has been varied with direct proportion to number of miner devices.
For example, the case containing 6 miners and 83 nodes difficulty of the PoW puzzle is assumed as $\alpha$, whereas for the case containing 12 miner and 166 nodes it is $2\alpha$.

To evaluate security in different block generation intervals, have generated two generation interval settings as 15 seconds and 1 minute.
For all evaluation cases,  we have fixed block size to 500 KB. 
We have used the Netherlands, Europe and World settings to simulate nodes' locations (see Section \ref{sec:settings}).
Evaluation results have been presented in Table \ref{tab:secEva2Neds}, \ref{tab:secEva2Europe} and \ref{tab:secEva2World}.
In which, we have presented number of genuine blocks, stale block generation rate and total work put into the blockchain.
We have calculated total work pun into the blockchain by multiplying number of genuine blocks with block generation difficulty.
...
..

Decreasing network latency among nodes cause to decrease stale block generation rates and helps to increase number of block generated.
Therefore for all evaluation cases, in general, the Netherlands settings has the longest blockchain and thus blockchains generated in this settings contain the most work.
As expected, in all cases, stale block rates are higher in 15 seconds block generation rate than 1 minute setting.
However as more blocks have been generated, for all cases blockchains generated in 15 seconds block generation interval setting includes more total work.
On the other hand, generally, blockchains with more devices tend to produce genuine blocks, due to higher stale block rates and less block generation (see Section \ref{sec:eva3}).
Even though such blockchains have less blocks especially with the 15 seconds block generation interval, they include more work due to higher block difficulty. 


The another important factor to consider is transaction throughput.
Indeed, for IoT environment achieving better transaction throughput is highly important. 
Shorter block generation intervals, i.e 15 seconds in our evaluations, increase the transaction throughput.
However, in short block generation intervals increasing number of devices participating in the blockchain significantly decreases number of genuine blocks.
We recall that we have set difficulty of the blockchains with direct proportion to the number of miner devices.
Thus, even though blockchains with higher difficulty put more work on the blockchain, their transaction throughput per second are significantly lower.
We can evaluate the throughput by just comparing number of genuine blocks, as block sizes have been fixed to 500 KB and all evaluations have been simulated for 100 minutes.
On 15 second block generation interval setting, transaction throughput of the evaluation cases containing 1250 devices are almost half of the evaluation cases containing 83 nodes.

Given all, we conclude that, if we consider a fixed block generation interval setting by varying difficulty according to block generation interval, decreasing number of devices in the blockchain cause blockchains to have less amount work, and be more vulnerable against attacks targeting it's integrity.
On the other hand, decreasing number of devices positively affect transaction throughput of blockchain, which is very important especially for it's scalability in the IoT domain.
In our architecture, we propose to use of consortium and private blockchains, which in turn make blockchain more robust against attacks targeting it's integrity (e.g. mining cartel attack presented in Section \ref{sec:51attack}).
Indeed, unlike public blockchains, malicious parties would not be able to directly connect to blockchain and take part in the consensus process.
That is said, we believe our architecture is advantageous considering performance and scalability of the blockchain systems on IoT domain, and with the use of private or consortium blockchains it does not generate big security vulnerability in contrast with decreasing total mining power.

.    



\begin{table}  
\begin{tabular} {|c|ccc|ccc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Interval:} & \multicolumn{3}{c}{\textbf{15 seconds}} & \multicolumn{3}{c}{\textbf{1 minute}} \\
\cmidrule(lr){2-4}  
\cmidrule(lr){5-7} 
\textbf{Results/} & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$}   & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$} \\
\textbf{Cases}	 & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}   & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}\\
\midrule
\textbf{6/83}   & 287.7&  7.15\% & 287.7$\alpha$      & 93.8  &1.57\% &93.8$\alpha$\\
\hline
\textbf{12/166} & 286.7&  13.25\% & 573.4$\alpha$	  & 92.4  &3.94\% &184.8$\alpha$\\ 
\hline
\textbf{18/250} & 264.7&  19.93\% &	794.1$\alpha$      & 97.6  &3.91\% &292.8$\alpha$\\ 
\hline
\textbf{36/500} & 200.9&  18.56\% &1205.4$\alpha$	  & 83.5  &4.02\% &501$\alpha$\\ 
\hline
\textbf{54/750} & 190.5&  17.12\% &1714.5$\alpha$	  & 81.0  &2.99\% &729$\alpha$\\ 
\hline
\textbf{72/1000}& 177.1&   18.2\% &2125.2$\alpha$	  & 97.6  &5.27\% &1171.2$\alpha$\\ 
\hline
\textbf{90/1250}&  162&   20.34\% &2430$\alpha$	      & 89.8  &3.21\% &1347$\alpha$\\ 
        \bottomrule             
\end{tabular}
\caption{Security evaluation \rom{2}: Netherlands setting} \label{tab:secEva2Neds} 
\end{table}


\begin{table}  
\begin{tabular} {|c|ccc|ccc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Interval:} & \multicolumn{3}{c}{\textbf{15 seconds}} & \multicolumn{3}{c}{\textbf{1 minute}} \\
\cmidrule(lr){2-4}  
\cmidrule(lr){5-7} 
\textbf{Results/} & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$}   & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$} \\
\textbf{Cases}	 & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}   & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}\\
\midrule
\textbf{6/83}   & 269.3 &  9.94\% & 269.3$\alpha$      & 98.3 &0\% &98.3$\alpha$\\ 
\hline
\textbf{12/166} &   273 & 16.87\% & 546$\alpha$	       & 90.6 &2.1\% &181.2$\alpha$\\ 
\hline
\textbf{18/250} & 234.4 & 19.3\% &	703.2$\alpha$      & 91.6 &8.6\% &274.8$\alpha$\\ 
\hline
\textbf{36/500} & 187.6 & 24.67\% & 1125.6$\alpha$	   & 91.3 &9.8\% &547.8$\alpha$\\ 
\hline
\textbf{54/750} & 173.1 & 19.95\% & 1557.9$\alpha$	  & 69.9 &12.9\% &629.1$\alpha$\\ 
\hline
\textbf{72/1000}& 162.6 & 23.34\% & 1951.2$\alpha$	  & 86.7 &11.0\% &1040.4$\alpha$\\ 
\hline
\textbf{90/1250}& 156.6 & 25.71\% & 2349$\alpha$	  & 77.8 &6.02\% &1166.9$\alpha$\\ 
\bottomrule             
\end{tabular}
\caption{Security evaluation \rom{2}: Europe setting} \label{tab:secEva2Europe} 
\end{table}



\begin{table}  
\begin{tabular} {|c|ccc|ccc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Interval:} & \multicolumn{3}{c}{\textbf{15 seconds}} & \multicolumn{3}{c}{\textbf{1 minute}} \\
\cmidrule(lr){2-4}  
\cmidrule(lr){5-7} 
\textbf{Results/} & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$}   & \multicolumn{1}{c}{$Genuine$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Total$} \\
\textbf{Cases}	 & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}   & \multicolumn{1}{c}{$Blocks$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$Work$}\\
\midrule
\textbf{6/83}   & 285.1 &  10.65\% & 285.1$\alpha$      & 100.3 &2.85\% &100.3$\alpha$\\ 
\hline
\textbf{12/166} & 233.5 & 22.82\% & 467$\alpha$	       & 88.2 &4.29\%  &166.4$\alpha$\\ 
\hline
\textbf{18/250} & 228.4 & 24.7\% &	685.2$\alpha$      & 79.2 &13.05\% &237.6$\alpha$\\ 
\hline
\textbf{36/500} & 181   &26.44\% &  1086$\alpha$	   & 95.4 & 8.79\% &572.4$\alpha$\\ 
\hline
\textbf{54/750} & 175.7 &22.58\% & 1581.3$\alpha$	   & 78.7 &10.21\% &708.3$\alpha$\\ 
\hline
\textbf{72/1000}& 155.3 &22.85\% & 1863.6$\alpha$	   & 80.8 & 12.4\% &969.6$\alpha$\\
\hline
\textbf{90/1250}& 156.7 &23.48\% & 2350.5$\alpha$	   & 71.1 &13.24\% &1066.5$\alpha$\\
\bottomrule             
\end{tabular}
\caption{Security evaluation \rom{2}: World setting} \label{tab:secEva2World} 
\end{table}











\iffalse

\textbf{Sending many valid transactions} 
%This DoS vector aims to overwhelm IoT device by increasing it's CPU usage, since peers of the blockchain networks have to check correctness of the transaction and if valid adding transaction to its memory. 
%We have emulated the victim IoT device and 10 attacker IoT devices with configurations given in Section \ref{sec:attackEmuStructure}. 
%In our experiments, attacker IoT devices continuously sent transactions directly to the victim device, the victim device has to check correctness of transactions and put into its memory if they are valid. 
%We have performed to attack for 30 minutes, where in total 65000 transactions with one input (attacker node's account address) and one output address, sent to the victim device. 
%We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:validTXs}, in which when attack started (around 15.01 in given figure) CPU usage increased significantly until attack has been terminated (around 15.31 in given figure). 
%As such, 10 attacker IoT devices with previously given configurations, in average, managed to consume 35\% of the CPU power of the victim IoT device. Additionally, such attack generated 16 MB overhead to RAM usage of the victim IoT device.

%In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. 
%In order to decrease possibility of successful attack, number of transactions that can be received from one peer in a period should be limited regrading resources of the IoT devices participating in the network. %Additionally, this attack comes with its cost in Bitcoin network, since attacker needs to pay transaction fee for each transactions, therefore applying a transaction fee can also reduce chances for successful attack. 




\textbf{Sending many invalid transactions} 
This DoS vector aims to overwhelm victim IoT device increasing its CPU usage. As such, we have evaluated this attack vector on Bitcoin network by continuously sending invalid transactions with one input and one output addresses, from 10 emulated attacker IoT devices to the victim IoT device. Attacker IoT devices continued to attack to the victim IoT device around 20 minutes, where we continuously send may invalid transactions. We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:invalidTXs}, in which when attack started (around 09.50 in given figure) CPU usage increased significantly until attack has been terminated (around 10.10 in given figure). In given configurations with 10 attacker nodes, in average, attacker devices managed to consume 53\% of the CPU power of the victim IoT device.

\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Invalid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with invalid TXs}
  \label{fig:invalidTXs} 
\end{figure}
In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. In order to decrease possibility of successful attack, connection to the peer that send invalid transactions should be dropped. 

\textbf{Sending many big transactions} 
This attack aims to cause memory overwhelm of victim IoT device, by sending many transactions that each are generating many outputs. We have tested this attack vector by  sending as many transactions as possible from one attacker IoT device with many output addresses to the victim IoT device on Bitcoin network which is configured with the settings given in Section \ref{sec:attackEmuStructure}. In our experiments, we have varied transaction sizes by varying number of output addresses in transactions. We present our results by showing number of outputs that we put in each transaction, size of the transaction, how many transactions with given settings could be sent to the peer and size of the total overhead on memory of the IoT device in Table \ref{tab:manyBigTX}. Bitcoin protocol drops the connection to the attacker node after receiving certain amount of transactions, which we executed many times every attack and presented the average number.
 
\begin{table}[t]
\centering
\caption{Generating Big Transactions}
\begin{tabular}{lllllll}
\hline
No of Output         & \multicolumn{1}{c}{100}  & \multicolumn{1}{c}{250}  & \multicolumn{1}{c}{500}  & \multicolumn{1}{c}{1000}  & \multicolumn{1}{c}{2000}  & \multicolumn{1}{c}{2950}  \\  \hline
TX Size (KB)             & \multicolumn{1}{c}{3.6}    & \multicolumn{1}{c}{8.7}   & \multicolumn{1}{c}{17.1}   & \multicolumn{1}{c}{34.2}   & \multicolumn{1}{c}{68.2}   & \multicolumn{1}{c}{98.8}    \\ \hline
No of TXs        & \multicolumn{1}{c}{296}  & \multicolumn{1}{c}{193}  & \multicolumn{1}{c}{108}  & \multicolumn{1}{c}{63}  & \multicolumn{1}{c}{32}  & \multicolumn{1}{c}{22}  \\  \hline
Total Size (MB)     & \multicolumn{1}{c}{1.06}  & \multicolumn{1}{c}{1.67}  & \multicolumn{1}{c}{1.86}  & \multicolumn{1}{c}{2.15}  & \multicolumn{1}{c}{2.18}  & \multicolumn{1}{c}{2.17}  \\  \hline
\end{tabular}
\end{table}\label{tab:manyBigTX}    
    

This attack may increase memory usage of IoT devices on the network, which may drop IoT devices from blockchain network by causing DoS. Therefore, in order to decrease success possibility of this attack vector, firstly maximum size of the transactions should be limited with regards to memory resource constraints of IoT devices on the network. Secondly, total size of the transactions that can be received from a peer should be limited, and connection to the peer should be dropped by victim peer device.
\fi


\iffalse
\subsection{Latency evaluation with Full Peers}
We have performed latency evaluation on our IoT architecture emulation, by measuring the time required for blockchain network starting from generation of release of transactions to achieving consensus state among IoT devices, about latest status of the blockchain. 
\textbf{Case 1: Varying blockchain sizes}  
We have evaluated effect of blockchain sizes to latency by varying number of peers in the blockchain network. In which, we have generated 4 different blockchains for our evaluation: with 20, 40, 100 and  200 IoT devices as blockchain peers. We have configured IoT devices with settings previously given in Section \ref{sec:emulationStructure}. We have put 500ms network delays between IoT devices, and Bitcoin protocol on IoT devices by generating connection among them with round-robin structure. In performing our evaluations, we set one of the IoT devices to generate 11000 transactions and release them to the blockchain network of our emulation's blockchain network. All transactions have same structure, where each one have one input and one output addresses and amount of Bitcoins to send to peer. After releasing transactions to the network, IoT device generated and released 5 blocks by one minute difference to previous one. 
Blockchain networks with more peers reaches to consensus in longer period. Network delays between nodes and block validation times plays a role in such behavior. Since network delay among IoT devices is fixed to 500 ms and block validations supposed to take same time since IoT devices configured to have same hardwares and block sizes are fixed. However, in our evaluations, latency does not increase proportional to network size, as presented in Table \ref{tab:latencyCase1}. As our evaluations showed, its better to decrease blockchain size to decrease latency, which obviously comes with a security trade-off which we discuss in detail at Section \ref{sec:security}.
\begin{table}[t]
\centering
\caption{Latency evaluation of case 1: Varying blockchain sizes}
\begin{tabular}{lllll}
\hline
                & \multicolumn{1}{c}{20 peers} &  \multicolumn{1}{c}{40 peers}  &  \multicolumn{1}{c}{100 peers} & \multicolumn{1}{c}{200 peers} \\ \hline
Latency         & \multicolumn{1}{c}{18 minutes}  & \multicolumn{1}{c}{20 minutes}  & \multicolumn{1}{c}{29 minutes} & \multicolumn{1}{c}{48 minutes}     \\ 
\end{tabular}
\end{table}\label{tab:latencyCase1}
\textbf{Case 2: Varying resources of IoT devices} We have varied amount resources that IoT devices have, which are acting as full peers of blockchain network, in order to test whether it effects latency of the system. In performing our evaluations, we have generated 4 different resource configurations given in Table \ref{tab:resources}\footnote{For CPU, given percentages presents assigned part of a single Power8 CPU with 3.5 GHz clock rate}, which has been applied to every IoT device in particular test case. In this test case, we have performed our evaluations with 40 IoT devices, and results have been presented in Table \ref{tab:latencyCase2}. Increasing amount of resources of IoT devices decreases block validation times, which decreased the time required for blockchain network to reach consensus state. 
\begin{table}[t]
\centering
\caption{Resource configurations}
\begin{tabular}{lllll}
\hline
                & \multicolumn{1}{c}{1st Conf} &  \multicolumn{1}{c}{2nd Conf}  &  \multicolumn{1}{c}{3rd Conf} & \multicolumn{1}{c}{4th Conf} \\ \hline
RAM         & \multicolumn{1}{c}{300 MB}  & \multicolumn{1}{c}{400 MB}  & \multicolumn{1}{c}{512 MB} & \multicolumn{1}{c}{1024 MB}     \\ \hline
CPU         & \multicolumn{1}{c}{1\%}  & \multicolumn{1}{c}{2\%}  & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%}     \\ 
\end{tabular}
\end{table}\label{tab:resources}

%$\frac{1}{4}$
\begin{table}[t]
\centering
\caption{Latency evaluation of case 2: varying resources of IoT devices}
\begin{tabular}{lllll}
\hline
                & \multicolumn{1}{c}{1st Conf} &  \multicolumn{1}{c}{2nd Conf}  &  \multicolumn{1}{c}{3rd Conf} & \multicolumn{1}{c}{4th Conf} \\ \hline
Latency         & \multicolumn{1}{c}{23 minutes}  & \multicolumn{1}{c}{21 minutes}  & \multicolumn{1}{c}{20 minutes} & \multicolumn{1}{c}{19.5 minutes}     \\ %\hline
\end{tabular}
\end{table}\label{tab:latencyCase2}
\fi
%To evaluate a lighter version of a blockchain protocol as an example to light peers of proposed architecture, we have used Bitcoin thin clients\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}. Bitcoin thin clients uses Simplified Payment Verification (SPV) protocol \footnote{$bitcoin.org/en/developer-guide\#simplified-payment-verification-spv$} for transaction verification without downloading whole blockchain and thin clients does not take part in consensus process or block generation of the blockchain network. We have used LXC system container tool to emulate light peers participating in blockchain network, that are configured to use Alpine Linux operating system\footnote{alpinelinux.org} version 3.6.0. Alpine Linux o.s. is a very lightweight and security oriented Linux distribution, which only requires around 5 MB of storage to set up using LXC tool. To develop example thin clients on Bitcoin network, we have used bitcoinj\footnote{bitcoinj.github.io} library, which is a bitcoin library that can be used with any JVM compatible language. We have set Java SE, JRE 8 update 131 environment to our light peers, and, we have developed Bitcoin thin client applications with bitcoinj library using Java SE, JDK version 8 Update 131. 
% In all of our experiments, we set RAM limit of light peers to the 64 MB, and limited CPU usage to 2\% of one core of Intel Core i7 2.70 GHz CPU. 
\iffalse
  \subfloat[CPU Utilization, 40 nodes, 2x CPU/RAM]{%
      \includegraphics[width=0.5\linewidth]{figures/40Nodes2x_CPU_Utilization.png}}
    \label{1c}\hfill   
&  \multicolumn{1}{c}{40 peers with 2x CPU/RAM}
&    \multicolumn{1}{c}{4.5\%}  
&   \multicolumn{1}{c}{127 MB}     
&   \multicolumn{1}{c}{6.7 KB/s}     
&    \multicolumn{1}{c}{8.7/s}        
\fi
%as following: RAMs of the IoT devices 128, 256, 512 and 1024 MB; and by varying their CPU usage 2\%, 3\%, 5\% and 10\%  respectively. 
%We have also evaluated latency and throughput of the blockchains on fixed size blockchains by changing amount of resources available for each peer of the blockchain network. 
%For this evaluation we have generated blockchains with 40 peers, where one of them is configured with 512 MB RAM and 5\% CPU usage limit for a peer as given above, and the other one is configured with 1 GB RAM and 10\% CPU usage limit. 
%As presented in Table \ref{tab:latencyCase2}, changing amount of resources assigned to the clients did not effect the latency or throughput of the blockchain network.
%Light client participation.
%However, before designing a blockchain with an alternative mining technique which allows all IoT devices to fairly participate in the system
%Similarly, as blockchains with less peers reaches consensus faster, they offer better throughout comparing to blockchains with more peers. 
%We discuss scalability in two dimensions: firstly latency and secondly throughput. Latency is discuss by average latency
%Finally, we have evaluated effect to of the resources of Bitcoin node to latency and performance. As such, we have doubled CPU (increased 5\% to 10\%) and RAM (increased 512 MB to 1 GB) of the blockchain with 40 clients and performed latency and performance evaluations with same settings given above.
\iffalse
\begin{table}[t]
\centering
\caption{Performance Statistics}
\begin{tabular}{lll}
\hline
                      & \multicolumn{1}{c}{Blockchain of 40 peers with doubled resources}    \\ \hline
Avg CPU usage         & \multicolumn{1}{c}{6\%}    \\
Avg RAM usage (active)& \multicolumn{1}{c}{184 MB}     \\
Avg Ethernet traffic  &  \multicolumn{1}{c}{6.7 KB/s}    \\
Avg Ethernet packets  &  \multicolumn{1}{c}{8.7/s}    \\
Avg Process Run Queue &   \multicolumn{1}{c}{7.1}   \\ \hline
\end{tabular}
\end{table}\label{tab:performanceResource}
\begin{figure} 
    \centering
  %\subfloat[CPU utilization with 2x resources, 40 nodes]{%      
     \includegraphics[width=\linewidth]{figures/40Nodes2x_CPU_Utilization.png}%}
  	%\label{1a}\\
  	%  \label{1a}\hfill
 % \subfloat[Blockchain with 100 nodes]{%
 %     \includegraphics[width=0.5\linewidth]{figures/40nodes_CPU_Utilization.png}}
%    \label{1b}\\
  \caption{CPU utilization of a peer with 2x CPU/RAM in blockchain with 40 nodes}
  \label{fig2} 
\end{figure}
\fi




DOS FIGURE PICTURE
\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Valid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with valid TXs}
  \label{fig:validTXs} 
\end{figure}



%\subsubsection{DoS Attack Evaluation}\label{sec:dosEvaluation}
%We have performed some Dos vectors targeting blockchain infrastructure by using Bitcoin protocol, and we have referred to Bitcoin stress test analysis in \cite{bitcoinStressTesting} for attack vectors. 
%We have performed 4 different DoS attack vectors on emulated IoT devices that participate in Bitcoin network. 
%In following, first we discuss our emulation settings then we present evaluated attacks and we discuss their their effects to the proposed architecture and how to protect against such attacks.

%\textbf{Dos attacks targeting blockchain infrastructure} 
%An attacker may perform DoS attack against blockchain infrastructure using her malicious blockchain nodes in the network. 
%Such attack is only effective against public blockchains, where anyone can participate in the network \footnote{We assume in private blockchains all peers are monitored closely by system administrators and if attacker compromise an IoT device and perform malicious activities, it can be detected easily and removed from the blockchain network}. 

%Attacker may target to cause unavailability of system, by preventing processing of transactions honest peers, or attacker may try to keep honest peers busy with his transactions to waste their resources thus interrupt correct execution of the blockchain network. As such, this attack may cause double spend transactions to succeed, may generate delays on block and transaction propagation or may prevent valid transactions to be mined into the new blocks.
%Second, in order to test performance of the light peers, we have simulated IoT devices with low resources.
%in which we set RAM limit of light peers to 64 MB, and limited CPU usage to 2\% of one core of Intel Core i7 2.70 GHz CPU. 
%We have used LXC system container tool to emulate light peers participating in blockchain network, that are configured to use Alpine Linux operating system\footnote{alpinelinux.org} version 3.6.0. 
%Alpine Linux o.s. is a very lightweight and security oriented Linux distribution, which only requires around 5 MB of storage to set up using LXC. 
%We have generated light peers in emulated IoT devices by using Bitcoin thin clients\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}. 
%Bitcoin thin clients use the Simplified Payment Verification (SPV) protocol \footnote{$bitcoin.org/en/developer-guide\#simplified-payment-verification-spv$} for transaction verification without downloading whole blockchain and they do not take part in  block generation or consensus process.  
%To develop example thin clients on Bitcoin network, we have used bitcoinj\footnote{bitcoinj.github.io} library, which is a bitcoin library that can be used with any JVM compatible language. 
%We have set Java SE, JRE 8 update 131 environment to our light peers, and, we have developed Bitcoin thin client applications with bitcoinj library using Java SE, JDK version 8 Update 131.




%We have to note that, we assume blockchain-IoT integration metrics defined in Section \ref{sec:metrics} have been adapted.
%There are two options to evaluate effects of the dividing mining power. 
%First is by fixing block generation interval according to number of devices in each scenario.
%and having four times shorter block generation interval in the scenario.
%However, applying this setting would not let to have a fair comparison of security of two scenarios, in that it simply is too much in favor to our proposed architecture.
%Indeed, as presented in Section \ref{sec:reqAnalysis}, increasing number of IoT devices and having a larger geographical area setting as devices' location increases stale block generation rates and blockchain-IoT metrics limits the stale block generation rates to $\approx$1\%.
%with regards to \textit{Confidentiality, Integrity} and \textit{Availability} (\textit{CIA}) triad, which have been widely used to classify capabilities and controls to achieve security outcomes in information security \cite{securityStandards}.
%There are different types of consensus issues, attacks targeting consensus of PoW blockchains (such as \cite{miningCartel,doubleSpending,misbehaviorInBitcoin}) 
%Therefore, in some sense, PoW blockchains' tamper-proof nature develops with generation of genuine blocks.
%\textbf{Confidentiality.}
%Fault tolerance, sonraki paper'a kaldi.
%\textbf{Availability.}
%Then we evaluate total amount of work each blockchain contains, and the one containing more work is more secure and robust to protect its integrity.
%The another important factor to consider is transaction throughput.
%Indeed, for IoT environment achieving better transaction throughput is highly important. 
%To this end, we evaluate how dividing blockchains effect security and whether can we compensate it or not.
%Particularly, we have generated two main security evaluations.
%On both of them, we have generated several evaluation cases containing different amount of IoT devices in different device location settings.
%In performing our first evaluation, we have assumed difficulty of the PoW puzzle is same for all evaluation cases. 
%Whereas in the second evaluation, we have varied difficulty of the PoW puzzle according to the number of devices for each evaluation case.
%We have performed our evaluations on the Bitcoin simulator presented in Section \ref{sec:simulator} by running the simulator 100 minutes for every evaluation case.
%Experiment results evaluated in Section \ref{sec:secEva1} and \ref{sec:secEva2}.
%Main motivation of using a blockchain architecture on IoT domain is to exploit strong robustness of blockchains and its tamper-proof nature.
%To this end, we quantitatively evaluate security of the proposed PoW based blockchain architecture with regards to \textit{Confidentiality, Integrity} and \textit{Availability} (\textit{CIA}) triad of the security objectives in information security and 
\iffalse
\noindent
\begin{tabular}{|l|*{6}{c|}}\hline
\backslashbox{\textbf{Settings}}{\textbf{Scenarios}} & \textbf{6 M} & \textbf{18 M} & \textbf{36 M} & \textbf{54 M} & \textbf{72 M} & \textbf{90 M} \\
             & \textbf{83 N} & \textbf{250 N} & \textbf{500 N} & \textbf{750 N} & \textbf{1000 N} & \textbf{1250 N} \\
         \hline
           \textbf{Hash} & & & & & & \\
           \textbf{Power} &  \textbf{10 MB} 	 & {\bf 10.82} 			& \textbf{0.00} 		 &{\bf 10.82}  			  &  {\bf 0.00\%}	 & {\bf 156.77s}   \\
            & & & & & & \\
       \hline
       \textbf{Block }   & & & & & & \\
          \textbf{Generation } &\textbf{5 MB}		 & {\bf 10.27}		    & \textbf{0.00}		     &{\bf 10.27}  			  &  {\bf 0.00\%} 	 & {\bf 78.35s}  \\		
        \textbf{Interval}   & & & & & & \\
        \hline
\end{tabular}
\fi
\iffalse
\noindent
\begin{tabular}{|@{\ $\bullet$\hspace*{3mm}}l||*{6}{c|}}\hline
\multicolumn{1}{|@{}l||}{\backslashbox{\textbf{Settings}}{\textbf{Scenarios}}}
& \textbf{6 M} & \textbf{18 M} & \textbf{36 M} & \textbf{54 M} & \textbf{72 M} & \textbf{90 M} \\
             & \textbf{83 N} & \textbf{250 N} & \textbf{500 N} & \textbf{750 N} & \textbf{1000 N} & \textbf{1250 N} \\
         \hline
           \textbf{Hash} & & & & & & \\
           \textbf{Power} &  \textbf{10 MB} 	 & {\bf 10.82} 			& \textbf{0.00} 		 &{\bf 10.82}  			  &  {\bf 0.00\%}	 & {\bf 156.77s}   \\
            & & & & & & \\
       \hline
       \textbf{Block }   & & & & & & \\
          \textbf{Generation } &\textbf{5 MB}		 & {\bf 10.27}		    & \textbf{0.00}		     &{\bf 10.27}  			  &  {\bf 0.00\%} 	 & {\bf 78.35s}  \\		
        \textbf{Interval}   & & & & & & \\
        \hline
&\makebox[3em]{5/31}&\makebox[4em]{6/1}&\makebox[3em]{6/2}
&\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
\end{tabular}
\bigskip
\fi
%\item \textbf{Sending very large blocks} Such attack vector may cause to generate bottlenecks on the network, as peers with constrained capabilities may fail to receive and propagate such blocks. Similarly to the above discussed attack vector, limiting block size will help to defend this attack vector.
%\subsection{Eclipse attack} 
%\subsection{Propagation delay attack} \label{sec:propagationDelay} By slowing down information propagation,. Propagation delay is the combination of transmission time and the local verification of the block or transaction w\cite{informationPropagation}. The goal of delay attack is to slow down the propagation of blocks towards or from a given set of nodes \cite{routingAttacks}.
%The scalability issues of the Bitcoin blockchain make it poorly suitable for the IoT, so we suggest to develop IoT applications on top of another secure but scalable blockchain. 
%In future work, we will test different blockchains to find a suitable one, in which the trade-off between scalability and security is acceptable. Moreover, we suggest to adopt a layered architecture which supports thin clients to allow IoT devices with limited resources to store only a portion of the blockchain.
%As discussed in \cite{securingIoT}, benefits of IoT could easily be suspended and outweighed by security vulnerabilities of it.  IoT is facing with serious security problems like identity management and encryption \cite{Whitmore2014}, access control and authentication \cite{sicariSecurity}. In \cite{learningIoTsecurity}, authors identified some of the most severe security and privacy threats for IoT as; leakage of personally identifiable information, leakage of sensitive user information and unauthorized execution of functions. Indeed, in addition to the foundational security concepts given above, privacy issues are very important for  IoT domain to gain wide acceptance among users. Privacy issues of IoT domain have been subject to extensive research in literature \cite{ourPaper, skarmeta, ourPaper2, odin}, and importance of privacy issues on IoT domain presented clearly.  
%Secondly such attack can be more effective by sending transactions with very small amounts, hence 
%Eavesdropping leads disclosure of data to perpetrator and thus harms privacy of the user. In contrast, since eavesdropping does not imply alteration of privacy meta-data, it does not imply damage to our mechanism. 
%In order for the transaction to be valid it has to have valid signatures from the public keys associated with the funds being transferred. It is regarded to be computationally unfeasible for a middleman to forge a signature if he does not possess the private key. These signatures are specific to the transaction and ensure its integrity, i.e., if the transaction is modified (by replacing recipient, amount, ...) then the signature becomes invalid.MITM: This would not work because the man in the middle's public key would not hash to the bitcoin address that owns the coins. What a man in the middle can do is perform a padding attack(malleability) which has largely been compensated for, but caused a lot of problems when it first came out. See more here
%Tampering threatens meta-data integrity by corrupting or altering data. Alteration of meta-data indeed is a serious threat for our mechanism, since privacy of the users is enforced according to the meta-data associated with the data.
%About tampering:In contrast, imagine a blockchain where every user can publish a hash associated to a particular file, OS image, software binary, or any other data which needs to be protected from tampering. While an attacker might be able to compromise the storage location and tamper with the data, they won’t be able to change the hash stored on the blockchain. This will make it known to everyone that the data has been manipulated. The difference between the blockchain security and traditional models is that, instead of relying on preserving secrets, the blockchain relies on transparency and general knowledge to protect information and data.
% Solution:  %To cope with these communication attacks, our framework can be  complemented with lightweight encryption mechanisms to secure data exchange among nodes, protect meta-data, and authenticate only valid smart objects for communication. Literature offers plenty of work dealing with such encryption mechanisms like \cite{lightweightAuthentication,cipherSecCertf,lightweightAuthSO}. In general, these solutions make use of lightweight cryptographic primitives (e.g., hash, nonce, etc), ensuring that data cannot be compromised during the communication.
%Proof of work requires expenditure of irretrievable resources to perform. Proof of work cannot be faked by spinning up more instances of the software, the energy actually has to be spent. In that sense PoW prevents Sybil attacks: even when an attacker isolates your node, they can only prevent you from getting updates from the network but not make you believe anything that the network hasn't actually agreed upon (unless they also sacrifice immense amounts of PoW).
%Similarly, when you run a full node for the first time you need to be able to connect to other nodes in the network to receive all the blocks that occured in the network so far. If by some chance your node connects to attacker's nodes they could try faking the transaction history. But since each block contains the difficulty at which it was mined, fake nodes being regular pc's or something like that would produce blocks at very low difficulties. If you ever connected to a real node, you would quickly discover that your node is under attack and receive the real history.
%The point is that if the fake nodes wanted to produce blocks at anything close to the current difficulty, they couldn't be just regular PC's and just fake the difficulty. They would have to be miners like the rest of the network, but then they are entering the race with other miners to produce blocks (or are trying to pull off a 51% attack).
%Sybil attacks are avoided in Bitcoin by requiring block generation ability to be proportional to computational power available through the proof-of-work mechanism. That way, an adversary is limited in how many blocks they can produce. This provides strong cryptographic guarantees of Sybil resilience.
%However, native Bitcoin mechanism provides an incentive to hide transactions, as nodes aware of transactions are compete to authorize first and claim the fee for authorization \cite{bitcoinAndRedBalloons}. In \cite{bitcoinAndRedBalloons}, authors proposed an incentive mechanism for nodes to broadcast transactions that they are aware of.
%Eclipse attack may be used for: block race attacks, generating forks thus splitting mining power, double spend attacks etc.
%In \cite{tamperingDelivery}, authors  showed that an adversary can exploit scalability measures (e.g. block size) in order to effectively delay the propagation of transactions and blocks to specific nodes, without causing network partitioning. 
%Since Bitcoin relies on a p2p network to track transactions, every transaction that node learns about should be transmitted to its neighbors in the network. 
% Tampering delivery of the blocks allows and causing delay allows adversary to easily mount DoS attacks, considerably increase its mining advantage in the network \cite{tamperingDelivery}. %Such attacks are even effective when a subset of the connections are intercepted \cite{routingAttacks}
%By delaying the propagation of blocks in the system, one can increase the amount of wasted blocks and proportionally slow down the growth of the longest branch of the system \cite{balanceAttack}. This delay presents a serious risk to the integrity of the blockchain, as the attacker does not even need a large fraction of the computational power to exceed the length of the chain, allowing her to double spend in new transactions the coins that she already spent in earlier transactions \cite{analysisDoubleSpending}. Additionally, this attack seriously threatens security of the PoW blockchains, since amount of works put in longest branch decreases.
%Specifically, attacker tries to delay propagation of newly generated blocks to a victim node or set of nodes without disrupting their connections. 
%Such attack may prevent participation of victim nodes from the blockchain network; may results as denial of service of the victim nodes; and may eclipse victim nodes.
%As such, this attack has two vectors as \textit{transaction hiding} and \textit{block withholding}.
%since theoretically he will be generating blocks more frequently than rest of the network so he will generate the longest blockchain, and eventually honest nodes will accept longest blockchain generated by attacker.
%We have implemented effects of such network partitioning attack using our Bitcoin testbed, to analyze vulnerabilities generated.
%Additionally, for blockchains using PoW consensus protocol, such attack causes decrease of total hash power of the blockchain network and decreases overall security provided by PoW consensus protocol. 
%By performing such attack vector, attacker interrupts execution of the blockchain network and perform malicious activities with bogus transactions and blocks.
%However, attacker can not force target IoT devices to accept something that network hasn't agreed upon before, without sacrificing huge amount of mining power by generating longer alternative blockchain. If somehow attacker manages to make victim believe his bogus blockchain, as soon as victim IoT device connects to honest node, it will discover the true history and recover, as long as attacker does not maintain majority of the mining power of the blockchain network.
%It will be impossible for hackers to circumvent the cryptography that makes the blockchain immutable, and there will be no single node they can compromise to publish their fake keys.
%effects of such attack vector has been discussed above at \textit{Propagation delay attack.}
%this attack aims to generate inconsistency inside blockchain network by trying to make peers having different views of current state of the blockchain, in order to perform malicious activities
%\item \textbf{Sending many invalid transactions} Such attack vector causes peer to perform a memory read to check whether process going to be performed by transaction complies with the current state of the blockchain. Such attack does not give an important overhead to the victim, since peer automatically declines the transaction after a memory read. To decrease effects of such attack on IoT devices with constrained resources, we propose use of a limit for receiving invalid transactions from a peer, device should drop out the connection when reaching the limit. 
%\item \textbf{Sending many valid transactions} Such attack aims to overwhelm cause memory and CPU overwhelm, since correctness of transactions first needs to be checked by peers and then must be added to memories of the blockchain peers before they sealed into blocks. To decrease effects of such attack, firstly number of the transactions kept in memories of peers should be limited with regards to memory capacities of IoT devices. Secondly, like previous attack vector, connection to a peer, that is sending many transactions maliciously, should be dropped. Moreover, if blockchain protocol requires attacker to pay fees to send transactions, this attack can be discouraged.
\iffalse
\begin{table}[t]
\centering
\caption{Latency evaluation of case 2: varying resources of IoT devices}
\begin{tabular}{lllll}
\hline
                & \multicolumn{1}{c}{} &  \multicolumn{1}{c}{ }  &  \multicolumn{1}{c}{ } & \multicolumn{1}{c}{ } \\ \hline
Latency         & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{ }  & \multicolumn{1}{c}{ } & \multicolumn{1}{c}{ }     \\ %\hline
\end{tabular}
\end{table}\label{tab:manyTXattackInvalid}
\fi
%In Bitcoin protocol, peer drops the connection to the peer that sends many invalid transactions. 
%In our evaluations, we have generated transactions that are sent from attacker to the victim peer, in which each transaction consists one input address, that is address of the attacker's account and another address. 
%We present results of our evaluations by presenting number of transactions send and whether connection dropped by the peer or not in Table \ref{tab:manyTXattackInvalid}. 
%In our evaluations, since connection is dropped by peer after XXX transactions, attacker could not overwhelm the peer.
%evaluated this attack vector on Bitcoin network by continuously sending transactions by developing an application using bitcoinj, discussed before.
%We present result of the such attack vector in Table \ref{tab:manyTXattackValid}.
		 %Firstly, Bitcoin protocol applies block size limit, which also implies a limit to the transactions since transactions must fit into the blocks. Therefore transactions with output addresses with 3000 or more address can not be generated, which indeed decreases overwhelm generated by a single transaction.
       %  We succeed to perform sending transactions with 2500 outputs, by targeting a fixed single peer of the network, and we kept constantly sending them. After performing several times same attack vector, on average, after 25 transactions peer that we target dropped the connection and did not accept anymore transaction. Which implies, on average, around 65KB of overload to the memory of peers. 
      %   Additionally, we have modified number of output addresses of a transactions, and tried to send them consequently to the peer. However, by using one client, we never managed to occupy more than 70KB of the memory of target peers, before connection dropped. 
      
      %Such attack vector aims to overwhelm CPU and memory of IoT devices on the blockchain network, since peers of blockchain network spend time to verify correctness of the transaction by using their CPU and they need to store correct transactions in their memory before they put in blocks. 
%In order to evaluate such, we have generated 
%As our findings show, Bitcoin network limits the maximum transaction size that can be generated by a peer. Therefore, such attack vector can be defended by limiting maximum transaction size, as all blockchain protocols limits the maximum transaction size. For proposed IoT architecture, transaction size should be limited with regards to networking capabilities of IoT devices acts as peers of the blockchain network.
%Proposed architecture exploits decentralized nature of blockchains to eliminates single point of failure of centralized systems to create more resilient system for IoT devices. 
%that tries to send more bitcoins than attacker account holds with 
%that are sent by 10 attacker IoT devices continuously.
%We have continued to attack to the victim IoT device around 20 minutes, where we constantly send may invalid transactions. 
%by configuring it with settings given in Section \ref{sec:attackEmuStructure}.
%This attack aims to cause memory overwhelm, by generating many outputs from one input. Indeed, such transaction occupies more space in memories of the peers, as all outputs needs to be kept in the memory of IoT devices until they have been used. This attack vector might be effective even limiting number of transactions that can be sent by a peer before killing connection differently from previous attack vectors, since many outputs generated by execution of a single transaction. 
